PREGO: online mistake detection in PRocedural EGOcentric videos

Promptly identifying procedural errors from egocentric videos in an online setting is highly challenging and valuable for detecting mistakes as soon as they happen. This capability has a wide range of applications across various fields, such as manufacturing and healthcare. The nature of procedural mistakes is open-set since novel types of failures might occur, which calls for one-class classifiers trained on correctly executed procedures. However, no technique can currently detect open-set procedural mistakes online. We propose PREGO, the first online one-class classification model for mistake detection in PRocedural EGOcentric videos. PREGO is based on an online action recognition component to model the current action, and a symbolic reasoning module to predict the next actions. Mistake detection is performed by comparing the recognized current action with the expected future one. We evaluate PREGO on two procedural egocentric video datasets, Assembly101 and Epic-tent, which we adapt for online benchmarking of procedural mistake detection to establish suitable benchmarks, thus defining the Assembly101-O and Epic-tent-O datasets, respectively.

==> sec/6_ablation.tex <==
\section{Ablation Study}
\LS{I've added parts from 6.1 directly in 5.2 and added a section 5.3 (the same as 6.2) as previously discussed, so that we could possibly remove this section.}
\label{sec:ablation}
Here, we present the results on step anticipation using two different Large Language Models (LLMs) (c.f. Sec. \ref{sec:which_LLM}) and compare them with the case of oracular step recognition (c.f. Sec. \ref{sec:oracol}). We also investigate the effect of different semantic prompts on the performance of the LLMs (c.f. Sec. \ref{sec:symbolic}). 








\subsection{Step Anticipation} 
\label{sec:which_LLM}


\paragraph{Llama Vs GPT-3.5}
In this section, we evaluate the performance of different LLMs for procedural mistake detection with symbolic inputs. We follow the Step Anticipation setting described in Sec. \ref{sec3:symb} and compare the LLAMA-2 model~\cite{touvron2023llama} with the OpenAI GPT-3.5 method. We report the results in Table \ref{tab:together}, using F1 score, precision and recall as the evaluation metrics. The Table shows that the OpenAI GPT-3.5 method achieves the highest F1 score on the \assemblyO dataset. We conclude that the OpenAI GPT-3.5 method is the most effective LLM for procedural mistake detection, as it can better learn the normal patterns of the procedures and detect deviations from them. We chose LLAMA as the LLM for the experiments on Epic-tent and the ablation studies due to its open source, accessible nature, and performance, which is almost on par with GPT-3.5.






\paragraph{Oracular Evaluation}
\label{sec:oracol}



To evaluate the action anticipation model's performance, we replace the step recognition branch's predictions with the ground truth action labels. This experiment mimics a situation where the video branch can perfectly recognize the actions performed in the videos. We refer to the last two rows in Table \ref{tab:together}, comparing them with PREGO and the other baseline methods. As expected, the oracle recognition experiment outperforms the PREGO model, achieving an F1 score of 46.3 and 44.1 with LLAMA and GPT-3.5, respectively, compared to 35.8 and 31.2 of PREGO, and indicating that the accuracy of the video branch is a bottleneck for the overall performance. However, the oracle recognition experiment also reveals our model's potential for improvement. Other factors influence the model's performance, such as the quality of the symbolic inputs, the semantic prompts, and the LLM architecture.
    
    


\subsection{Performance of different prompt types }
\label{sec:symbolic}

We investigate the effect of different action representations in the prompt for the Step Anticipation prediction. Following \cite{generalpatternmachines2023}, we consider three ways of representing an action: numerical, semantic, or random symbols. Numerical representation means that an action label is replaced with an index in the range $[0,\mathcal{A}]$, where $\mathcal{A}$ is the total number of actions. Semantic representation implies that the action is represented by its action label. Random symbol indicates that each action is assigned to a different symbol, such as a set of emojis. This allows us to examine how the LLM can manage different levels of abstraction and expressiveness of the input prompt. Fig. \ref{fig:frame_pic} illustrates an example of a prompt in the three different representations. 
\input{Tables/symbolic_input}

Table \ref{tab:symbolic} shows the experiment results using the described representations. We observe that all the different representations achieve
%assumes 
close performance, with the numerical representation achieving the highest F1 score, with 33.4, followed by the random representation, 33.2. We hypothesize that the numerical representation is easier for the model to understand and predict the next step, as it reduces the number of tokens to be generated. Indeed, an action index requires only four tokens, whereas the emojis and the action labels require at least eight tokens. 
Remarkably, the semantic representation achieves a comparable performance even though words can introduce bias or ambiguity into the model. This indicates that the model can handle the natural language input and extract the relevant information for the step anticipation task. 
Surprisingly, the random symbol representation has a comparable performance to the other representations, even though the model does not have any semantic or numerical association with them. This suggests that the model can learn the temporal structure of the actions from the input history, regardless of the symbol representation. 



==> sec/Backup/0_abs_2023-11-05.tex <==
\begin{abstract}
\AL{
The increase in the use of Augmented Reality (AR) and Virtual Reality (VR) systems, particularly in industries such as healthcare and manufacturing, requires the development of robust systems for accurate procedure assessment. We propose a novel method for mistake detection in procedural egocentric videos, taking into account the open-setness of mistakes, which means that never-seen-before anomalies can occur after training. \LS{Possible rephrasing: We propose an innovative approach for detecting errors in procedural egocentric videos, considering the challenge of open-set mistakes, where previously unseen anomalies may occur post-training.} Inspired by recent anomaly detection techniques, we propose a one-class classification method, where the model is trained only on procedures without mistakes, committed to learning the correct procedures workflows.
\LS{Possible rephrasing: we propose a one-class classification approach in which the model exclusively trains on mistake-free procedures, focusing on learning the accurate procedure workflows.}
Furthermore, we explore the ability of Large Language Models (LLMs) in addressing logical challenges within unknown contexts. This encompasses evaluating their zero-shot capabilities and measuring their effectiveness in scenarios they were not explicitly trained for, specifically focusing on mistake detection.
\LS{Possible rephrasing: Moreover, we investigate the potential of Large Language Models (LLMs) to tackle logical challenges in unfamiliar contexts and leverage their reasoning abilities. This includes assessing their zero-shot capabilities and measuring their performance in contexts where they were not explicitly trained, specifically focusing on detecting errors.}
We evaluate our proposed methodology using two benchmark datasets: Assembly101 and EpicTent.
}

% \AL{from the project proposal doc:\\
% We propose a novel model and a benchmarking protocol for the problem of online Procedural Mistake Detection (PMD) in egocentric videos. Our contributions are threefold: firstly, we introduce PMD in multiple domains such as manufacturing and healthcare, where procedure accuracy is paramount. Secondly, we perform online PMD for error detection and prevention, which is particularly valuable in egocentric video contexts. Thirdly, similar to anomaly detection approaches, we utilize the one-class classification paradigm, eliminating the need for mistake labels, enhancing our method's self-supervised learning capacity, and reducing dependence on labeled data. In summary, our research advances egocentric PMD, ensures timely error identification, and enhances self-sufficiency in learning from unannotated data.
% }

\end{abstract}

==> sec/Backup/0_abs_2023-11-09.tex <==
\begin{abstract}
% In industries such as healthcare and manufacturing, the recognition of egocentric action videos promotes safety via the online recognition of procedural mistakes. 
% \AF{I would rephrase: 
Recognizing procedural mistakes from egocentric videos in an online setting has applications in different domains, including manufacturing and healthcare.
% }
Mistakes are open-set, as novel unforeseen failures may occur, and should be detected in due course. \AL{Moreover, mistakes are also open-class since it is difficult to obtain labeled data for all possible types of errors, and asking subjects to fail on purpose to train supervised models is not a practical option.}
\AF{Also, it could be worth mentioning that, apart from being open-set, they are open class - it's hard to label mistakes and in an industrial process, we cannot ask subjects to purposedly make mistakes so that we can train supervised methods.}
%\ED{Isn't that what we're already stating? Train and evaluation sets do not necessarily share the same label space, so we train on some classes and may test on never-seen ones.}
%\AL{@edo one-class and open-set refer to the mistakes in this case, not the different set of classes that are present in train and test. }
Although a growing number of works focus on the topic, no model currently meets these requirements, nor has a benchmark been devised for the specific goal. 
%\FG{check the statement}

We propose PREGO, the first one-class \AF{(online?)} classification model for mistake detection in procedural egocentric videos. 
First, we revise two popular egocentric video datasets, ASSEMBLY101 and EpicTents, containing labeled mistakes, to define suitable benchmarks, i.e.\ setting the goal as detecting the first occurrence of the mistake online, out of training on correct procedures just. \AL{in the case of Assembly this sentence is 100\% right. In EpicTents --almost-- all the videos have mistakes. We create the splits based on the confidence of the actor. In some scenarios could be difficult to see if every frames are correct, so we need to trust the confidence of the actor.}
Then, we align a state-of-the-art egocentric video recognition model with symbolic reasoning over the label space. 
The first recognizes the current action; the second predicts the expected action based on the accomplished prior procedure. \AL{I'd push more on explaining why we choose symbolic reasoning.} 
Mistakes are detected by misalignments, a viable path, as we demonstrate on ASSEMBLY101 and EpicTents. \AL{we already mentioned the datasets. Should we restate it here?}


%\FG{Previous version commented, also saved in a backup tex screenshot in the backup folder.}
% \AL{
% The increase in the use of Augmented Reality (AR) and Virtual Reality (VR) systems, particularly in industries such as healthcare and manufacturing, requires the development of robust systems for accurate procedure assessment. We propose a novel method for mistake detection in procedural egocentric videos, taking into account the open-setness of mistakes, which means that never-seen-before anomalies can occur after training. \LS{Possible rephrasing: We propose an innovative approach for detecting errors in procedural egocentric videos, considering the challenge of open-set mistakes, where previously unseen anomalies may occur post-training.} Inspired by recent anomaly detection techniques, we propose a one-class classification method, where the model is trained only on procedures without mistakes, committed to learning the correct procedures workflows.
% \FG{I'm missing the motivation for introducing our work}
% \LS{Possible rephrasing: we propose a one-class classification approach in which the model exclusively trains on mistake-free procedures, focusing on learning the accurate procedure workflows.}
% Furthermore, we explore the ability of Large Language Models (LLMs) in addressing logical challenges within unknown contexts. This encompasses evaluating their zero-shot capabilities and measuring their effectiveness in scenarios they were not explicitly trained for, specifically focusing on mistake detection.
% \LS{Possible rephrasing: Moreover, we investigate the potential of Large Language Models (LLMs) to tackle logical challenges in unfamiliar contexts and leverage their reasoning abilities. This includes assessing their zero-shot capabilities and measuring their performance in contexts where they were not explicitly trained, specifically focusing on detecting errors.}
% \FG{Fine to mention LLMs, but better to talk about reasoning in the action label space (which can be done with llms in various ways) and comparing the result with video recognition}
% We evaluate our proposed methodology using two benchmark datasets: Assembly101 and EpicTent.
% }


% \AL{from the project proposal doc:\\
% We propose a novel model and a benchmarking protocol for the problem of online Procedural Mistake Detection (PMD) in egocentric videos. Our contributions are threefold: firstly, we introduce PMD in multiple domains such as manufacturing and healthcare, where procedure accuracy is paramount. Secondly, we perform online PMD for error detection and prevention, which is particularly valuable in egocentric video contexts. Thirdly, similar to anomaly detection approaches, we utilize the one-class classification paradigm, eliminating the need for mistake labels, enhancing our method's self-supervised learning capacity, and reducing dependence on labeled data. In summary, our research advances egocentric PMD, ensures timely error identification, and enhances self-sufficiency in learning from unannotated data.
% }

\end{abstract}

==> sec/Backup/0_abs_2023-11-12.tex <==
\begin{abstract}

Promptly identifying procedural errors from egocentric videos in an online environment is highly valuable for detecting mistakes as they happen. This capability has a wide range of applications across various fields, such as manufacturing and healthcare.
The nature of mistakes is open-set,
\FG{rephrase all rest of this paragraph with this text only: "since novel types of failures might occur, which calls for one-class classifiers trained on correctly executed actions. However, no technique can currently detect open-set procedural mistakes online." We need to end the first paragraph with a criticism which our model fixes/proposes as novlety.}
acknowledging the potential for novel, unforeseen failures that require timely identification. In real-world scenarios, mistakes also demonstrate a one-class characteristic, as obtaining labeled data for all possible error types proves challenging. Intentionally inducing failures in subjects for supervised model training is often impractical.
% \AL{Moreover, mistakes are also open-class since it is difficult to obtain labeled data for all possible types of errors, and asking subjects to fail on purpose to train supervised models is not a practical option.}
% \AF{Also, it could be worth mentioning that, apart from being open-set, they are open class - it's hard to label mistakes and in an industrial process, we cannot ask subjects to purposedly make mistakes so that we can train supervised methods.}
%  \FG{I'm also a bit puzzled on the open class. Mentioning that labelling is hard is a praise to ASSEMBLY101, not a point relevant to this paper.}

\FG{The current start of the second paragraph is correct, but not directly stating the reason why we make this paper for, our main contribution. I had proposed this text "We propose PREGO, the first online one-class classification model for mistake detection in procedural egocentric videos." This may be wrong, but I meant to pin point that we need to state very clearly our main contributions straightaway, our right to make a paper.} As a One-Class Classification (OCC) model, our model PREGO is designed to recognize errors in videos that the actor considers correct and to categorize any unexpected open-set procedures as mistakes.
To achieve this, we \FG{.."we resort to two widely.."}draw samples from two widely used egocentric video datasets, ASSEMBLY101 and EpicTents, \FG{repetition, remove the next words, and add "which we rearrange for OCC learning and for online benchmarking of procedural mistakes". In fact, we do not need "OCC learning", as nothing is specific in the benchmarks for it, right? so only keep the "online benchmarking"}to establish suitable benchmarks. Specifically, our objective is to detect the initial instance of a mistake in real-time, having trained the model solely on correct procedures. \LS{As pointed out by Ale, this is not completely true. How should we phrase it?}
\FG{This sentence contains a few bugs. Real-time is wrong. Correct procedures is a repetition of OCC. In fact, I'd remove the sentence. The only needed part is the reference to the first mistake, but it's not clear why is so. So my proposition for considering online benchmarking.}
% \AL{in the case of Assembly this sentence is 100\% right. In EpicTents --almost-- all the videos have mistakes. We create the splits based on the confidence of the actor. In some scenarios could be difficult to see if every frames are correct, so we need to trust the confidence of the actor.}
PREGO incorporates two distinct branches. The first \FG{remove "branch"}branch classifies the current action using a video action recognition model. \FG{remove "in contrast"}In contrast, the second anticipates the\FG{this} action by harnessing the capabilities of Large Language Models (LLMs) for symbolic reasoning across the label space\FG{rephrase the rest of this paragraph: ". PREGO detects procedural mistakes online when recognition and anticipation do not align, demonstrating robustness to multiple plausible ways of accomplishing a procedure, and considering dependencies within complex activities."} in a zero-shot manner. It accounts for various ways of completing a procedure and the intricate dependencies within complex activities.

% We propose PREGO, the first online one-class classification model for mistake detection in procedural egocentric videos. 
% First, we revise two popular egocentric video datasets, ASSEMBLY101 and EpicTents, containing labeled mistakes, to define suitable benchmarks, i.e.\ setting the goal as detecting the first occurrence of the mistake online, out of training on correct procedures just. \FG{maybe explain why we do this,  start this sentence by setting the motivation for it, eg "Being OCC, our model learns on correct videos just (or what the actor considers so) and detects as mistaken any unexpected (open-set) procedure. So we sample from two popular egocentric video datasets, ASSEMBLY101 and EpicTents, excerpts without any mistake, from the start of the procedures"}
% \AL{in the case of Assembly this sentence is 100\% right. In EpicTents --almost-- all the videos have mistakes. We create the splits based on the confidence of the actor. In some scenarios could be difficult to see if every frames are correct, so we need to trust the confidence of the actor.}
% Then, we align a state-of-the-art egocentric video recognition model with symbolic reasoning over the label space. 
% The first recognizes the current action; the second predicts the expected action based on the accomplished prior procedure \FG{and all similar training examples.}. \AL{I'd push more on explaining why we choose symbolic reasoning.}\FG{yes, I agree, this part is interesting and very timely in the field. Maybe: "Next action prediction leverages large language models, employed for symbolic reasoning zero-shot'ly, to account for multiple pathways of accomplishing a procedure and the complex activity dependencies." or something similar. maybe too long.} 
\FG{remove:}The promising results we obtain stem from our approach of identifying procedural errors through misalignment.
% Mistakes are detected by misalignments, a viable path, as we demonstrate on ASSEMBLY101 and EpicTents. \AL{we already mentioned the datasets. Should we restate it here?}\FG{here it's for saying results are good enough.. can avoid repeating the datasets but needs to add something about the promising quality.} 


\end{abstract}

==> sec/Backup/0_abs_2023_11-09_sec.tex <==
\begin{abstract}
% In industries such as healthcare and manufacturing, the recognition of egocentric action videos promotes safety via the online recognition of procedural mistakes. 
% \AF{I would rephrase: 
Recognizing procedural mistakes from egocentric videos in an online setting has applications in different domains, including manufacturing and healthcare.
% }
Mistakes are open-set, as novel unforeseen failures may occur, and should be detected in due course. \AL{Moreover, mistakes are also open-class since it is difficult to obtain labeled data for all possible types of errors, and asking subjects to fail on purpose to train supervised models is not a practical option.}
\AF{Also, it could be worth mentioning that, apart from being open-set, they are open class - it's hard to label mistakes and in an industrial process, we cannot ask subjects to purposedly make mistakes so that we can train supervised methods.}
%\ED{Isn't that what we're already stating? Train and evaluation sets do not necessarily share the same label space, so we train on some classes and may test on never-seen ones.}
%\AL{@edo one-class and open-set refer to the mistakes in this case, not the different set of classes that are present in train and test. }
\FG{I'm also a bit puzzled on the open class. Mentioning that labelling is hard is a praise to ASSEMBLY101, not a point relevant to this paper.}
Although a growing number of works focus on the topic, no model currently meets these requirements \FG{maybe here repeat for clarity, eg "the online and openset requirements"}, nor has a benchmark been devised for the specific goal. 
%\FG{check the statement}

We propose PREGO, the first one-class \AF{(online?)}\FG{yes, online to add.} classification model for mistake detection in procedural egocentric videos. 
First, we revise two popular egocentric video datasets, ASSEMBLY101 and EpicTents, containing labeled mistakes, to define suitable benchmarks, i.e.\ setting the goal as detecting the first occurrence of the mistake online, out of training on correct procedures just. \FG{maybe explain why we do this,  start this sentence by setting the motivation for it, eg "Being OCC, our model learns on correct videos just (or what the actor considers so) and detects as mistaken any unexpected (open-set) procedure. So we sample from two popular egocentric video datasets, ASSEMBLY101 and EpicTents, excerpts without any mistake, from the start of the procedures"}
\AL{in the case of Assembly this sentence is 100\% right. In EpicTents --almost-- all the videos have mistakes. We create the splits based on the confidence of the actor. In some scenarios could be difficult to see if every frames are correct, so we need to trust the confidence of the actor.}
Then, we align a state-of-the-art egocentric video recognition model with symbolic reasoning over the label space. 
The first recognizes the current action; the second predicts the expected action based on the accomplished prior procedure \FG{and all similar training examples.}. \AL{I'd push more on explaining why we choose symbolic reasoning.}\FG{yes, I agree, this part is interesting and very timely in the field. Maybe: "Next action prediction leverages large language models, employed for symbolic reasoning zero-shot'ly, to account for multiple pathways of accomplishing a procedure and the complex activity dependencies." or something similar. maybe too long.} 
Mistakes are detected by misalignments, a viable path, as we demonstrate on ASSEMBLY101 and EpicTents. \AL{we already mentioned the datasets. Should we restate it here?}\FG{here it's for saying results are good enough.. can avoid repeating the datasets but needs to add something about the promising quality.} 

%\FG{Previous version commented, also saved in a backup tex screenshot in the backup folder.}
% \AL{
% The increase in the use of Augmented Reality (AR) and Virtual Reality (VR) systems, particularly in industries such as healthcare and manufacturing, requires the development of robust systems for accurate procedure assessment. We propose a novel method for mistake detection in procedural egocentric videos, taking into account the open-setness of mistakes, which means that never-seen-before anomalies can occur after training. \LS{Possible rephrasing: We propose an innovative approach for detecting errors in procedural egocentric videos, considering the challenge of open-set mistakes, where previously unseen anomalies may occur post-training.} Inspired by recent anomaly detection techniques, we propose a one-class classification method, where the model is trained only on procedures without mistakes, committed to learning the correct procedures workflows.
% \FG{I'm missing the motivation for introducing our work}
% \LS{Possible rephrasing: we propose a one-class classification approach in which the model exclusively trains on mistake-free procedures, focusing on learning the accurate procedure workflows.}
% Furthermore, we explore the ability of Large Language Models (LLMs) in addressing logical challenges within unknown contexts. This encompasses evaluating their zero-shot capabilities and measuring their effectiveness in scenarios they were not explicitly trained for, specifically focusing on mistake detection.
% \LS{Possible rephrasing: Moreover, we investigate the potential of Large Language Models (LLMs) to tackle logical challenges in unfamiliar contexts and leverage their reasoning abilities. This includes assessing their zero-shot capabilities and measuring their performance in contexts where they were not explicitly trained, specifically focusing on detecting errors.}
% \FG{Fine to mention LLMs, but better to talk about reasoning in the action label space (which can be done with llms in various ways) and comparing the result with video recognition}
% We evaluate our proposed methodology using two benchmark datasets: Assembly101 and EpicTent.
% }


% \AL{from the project proposal doc:\\
% We propose a novel model and a benchmarking protocol for the problem of online Procedural Mistake Detection (PMD) in egocentric videos. Our contributions are threefold: firstly, we introduce PMD in multiple domains such as manufacturing and healthcare, where procedure accuracy is paramount. Secondly, we perform online PMD for error detection and prevention, which is particularly valuable in egocentric video contexts. Thirdly, similar to anomaly detection approaches, we utilize the one-class classification paradigm, eliminating the need for mistake labels, enhancing our method's self-supervised learning capacity, and reducing dependence on labeled data. In summary, our research advances egocentric PMD, ensures timely error identification, and enhances self-sufficiency in learning from unannotated data.
% }

\end{abstract}

==> sec/Backup/1_intro_2023-11-05.tex <==
\section{Introduction}
\TD{Sketch of intro
\begin{itemize}
    \item using bullets
    \item This shows the flow of the main argument for problem motivation, what’s missing in related work, and the claimed novelty
\end{itemize}}
\label{sec:intro}
\GD{\begin{enumerate}
    \item There is a rising interest in procedure learning due to advancements in Augmented Reality (AR) and Virtual Reality (VR).
    \item Besides facilitating procedure learning, these technological devices also optimize workflow in real-time.
    \item For instance, a device could assist a human operator by evaluating the correctness of a procedure in real-time and offering immediate suggestions to correct any errors made.
    \item Recently, numerous studies have introduced datasets and methods focused on procedure learning and error detection within industrial contexts.
    \item However, there is a lack of methods aimed at detecting errors in procedural egocentric videos. The existing literature is scattered and fragmented, with varied metrics and experiments, making comparisons between recently proposed methods challenging.
    \item This disparity is likely due to the highly specific nature of procedures and the rarity and labeling difficulty of mistakes, similar to anomalies in real-life scenarios.
    \item Inspired by these challenges, this paper introduces a novel method to identify errors in procedural egocentric videos by learning exclusively from correct procedures and detecting mistakes when operator actions deviate from network expectations.
    \item Description of the double-branch architecture:
    \begin{itemize}
        \item \textit{Action-recognition branch:} Analyzes frames in a procedural video up to time \(t\) and predicts the current action performed by the operator.
        \item \textit{Action-anticipation branch:} Compiles the sequences of predicted actions up to time \(t-1\) and forecasts the subsequent action to be executed.
        \item An error is detected when there is a discrepancy between the recognized action and the action anticipated by the predictor.
    \end{itemize}
    \item The action-anticipation branch can be configured in multiple ways. For example, it could operate as a video stream that processes a shorter context than the "current branch," focusing on forecasting the imminent action rather than recognizing it.
    \item However, this approach may not fully leverage the intrinsic nature of procedures, which fundamentally revolve around the sequential patterns of actions leading to the completion of a process.
    \item Recognizing this and inspired by recent advancements in Symbolic reasoning, we propose the adoption of an LLM. This model aims to comprehend and synthesize the procedural patterns of actions to predict subsequent actions accurately.
    \item The LLM considers the sequence of recognized actions within a procedure and incorporates context from related procedures. It utilizes a symbolic representation of action sequences, enhancing the forecasting accuracy of the upcoming actions in the procedural flow.
\end{enumerate}}

\LS{The bullet points perfectly summarize the work. However, at some points, I would add the reasoning's capability of LLMs which justifies its usage in this work.}
\GD{yes, I was searching for the right way to include it. I did it describing the prediction branch, but maybe one can spend more words describing a procedure, its symbolic Vs. semantic representation and then introduce the LLM branch}
\ED{I'd directly speak of the \textit{action-anticipation} with LLMs, moving points 9 and 10 to (i) the related works, in a paragraph for video-based techniques, or (ii) in the methodology, right after the \textit{action-recongition} branch, distancing ourselves from OadTR}

\input{Tables/comparison_with_sota}
\input{Tables/video-based}
\input{Tables/LLM}

==> sec/Backup/1_intro_2023-11-07.tex <==
\section{Introduction} \label{sec:intro}
% \TD{Sketch of intro
% \begin{itemize}
%     \item using bullets
%     \item This shows the flow of the main argument for problem motivation, what’s missing in related work, and the claimed novelty
% \end{itemize}}

\begin{enumerate}
    \item There is a rising interest in procedure learning due to advancements in Augmented Reality (AR) and Virtual Reality (VR).
    \item Besides facilitating procedure learning, these technological devices also optimize workflow in real-time. \AF{I think this point could be removed.}
    \item For instance, a device (\AF{an AR device?)} could assist a human operator by evaluating the correctness of a procedure in real-time and offering immediate suggestions to correct any errors made.
    \item Recently, numerous studies have introduced datasets and methods focused on procedure learning and error detection within industrial contexts.
    \item However, there is a lack of methods (\AF{investigations?}) aimed at detecting errors in procedural egocentric videos. The existing literature is scattered and fragmented, with varied metrics and experiments, making comparisons between recently proposed methods challenging. \FG{It isn't true that mistake detection is not done, right? It isn't done online. Fragmentation might be a point. But a better one is to say: we want requirements of open-set'ness and online. And there isn't any method. In fact, there isn't any benchmark either. Here I'd conclude the first paragraph. From the next, we make our proposal.} \AL{we can also think to answer the possible questions of the reviewer "Why using LLMs instead of video-based anomaly detection (VAD) techniques?" The setup we're proposing has a limited set of normal procedure, instead VAD methods learn normality from a huge number of normal samples. The symbolic reasoning of LLMs is then a possible answer to this problem. }\AF{I agree with Fabio: It would be great to take a SoA method for VAD and show its limitations. I agree with highlighting the online bit, but I also like the argument that ``literature is scattered''.}
    \item This disparity is likely due to the highly specific nature of procedures and the rarity and labeling difficulty of mistakes, similar to anomalies in real-life scenarios.\FG{This may be omitted}
    \item \FG{Start of the second paragraph} Inspired by these challenges, this paper introduces a novel method to identify errors in procedural egocentric videos by learning exclusively from correct procedures \AF{(How does this align to the discussion we had on slack on the new split which would technically contain unlabeled mistakes in the training set? - what about saying that we learn from videos in which mistakes are not labeled?)} and detecting mistakes when operator actions deviate from network expectations \FG{online}.
    \item \FG{This may be a third paragraph, the proposed procedure}Description of the double-branch architecture:
    \begin{itemize}
        \item \textit{Action-recognition branch:} Analyzes frames in a procedural video up to time \(t\) and predicts the current action performed by the operator. \FG{This leverages the SOTA video-based online action recognition OadTR.}
        \item \textit{Action-anticipation branch:} Compiles the sequences of predicted actions up to time \(t-1\) and forecasts the subsequent action to be executed. \FG{This is based on symbolic reasoning over the label space, formulated as zero-shot next action label prediction, assuming the context of correct procedures, in LLAMA and GPT-4.}
        \item An error is detected when there is a misalignment between the recognized action and the action anticipated by the predictor.
    \end{itemize} 
    % \FG{terminate here the second paragraph}
    \item \FG{Start here the fourth paragraph} There is no suitable benchmark. There is data of labelled mistakes, but videos proceed after the mistake, so detecting disassembly means detecting mistakes \GD{I didn't get this last sentence}. \AF{I don't know if this is actually worth mentioning. In an online scenario, in some sense, it does not matter, as you will not get to see the ``detach'' actions} Also, procedures after the mistakes are altered. We need to consider procedures, to stop at the first mistake. Ideal is open-set'ness. etc \FG{tentative text, describing our proposed revision of the assembly101 and epictent benchmarks} \AF{What about something like ``While Assembly101 has been designed to tackle supervised, off-line mistake detection, we consider an online scenario in which the user is notified as soon as the mistake is recognized. Hence, rather than considering all labeled mistakes, we focus on the first mistake happening in each video. - verbose, not suggesting to take it verbatim}
    \item \FG{Start a fifth paragraph on the in-depth analysis, via oracles and ablative studies, incl BERT etc} The action-anticipation branch can be configured in multiple ways. For example, it could operate as a video stream that processes a shorter context than the "current branch," focusing on forecasting the imminent action rather than recognizing it. \AF{What about posing it as ``We investigate different configurations for the anticipation branch ...''}
    \item However, this approach may not fully leverage the intrinsic nature of procedures, which fundamentally revolve around the sequential patterns of actions leading to the completion of a process.
    \item Recognizing this and inspired by recent advancements in Symbolic reasoning, we propose the adoption of an LLM. This model aims to recognize and synthesize the procedural patterns of actions to predict subsequent actions accurately. \FG{Into the third paragraph?}
    \item The LLM considers the sequence of recognized actions within a procedure and incorporates context from related procedures. It utilizes a symbolic representation of action sequences, enhancing the forecasting accuracy of the upcoming actions in the procedural flow. \FG{Into the third paragraph?}
    \item \FG{Sixth final paragraph} On both benchmarks the performance is not perfect, but it's a very valid first step.
\end{enumerate}

\FG{The previous bullet list is saved in the backup folder file. I've iterated on the existing valid one, altered the numbers a bit. In general, refer to paragraphs, we'll need those too.}\\
\GD{Egocentric view is not stressed enough; the connection with our work is in the use-case: a worker wearing an AR device while working gets recommendations and corrections in real-time since the AR device online analyzes his actions and movements.}

Procedure learning is garnering considerable interest due to the advancements in Augmented Reality (AR) and Virtual Reality (VR) technologies. 
These innovations are not only pivotal for enhancing procedural knowledge and skill acquisition but also play a crucial role in streamlining workflow efficiencies in real-time applications.
For instance, AR and VR devices can aid human operators by providing instantaneous feedback on the accuracy of their performed tasks, thereby enabling immediate corrective actions.
Recent works have yielded a multitude of datasets~\cite{epicTent,IndustReal,sener2022assembly101,HoloAssist2023,ghoddoosian2022weakly,ding2023every,coin,ikea,IndustReal,cross_task,proceL_2019,howto100m_2019_miech} and methodologies aimed at advancing procedure learning~\cite{POC_2022,ghoddoosian2022weakly,OadTR,zhong_2023,epicTent,coin} and error detection~\cite{HoloAssist2023,ding2023every,IndustReal}, particularly within industrial environments. 
Despite these advancements, the current literature reveals a lack of frameworks capable of detecting errors in procedural egocentric videos for industry applications in an online fashion.
Indeed, current approaches typically focus on specific types of errors e.g., detecting the wrong order of steps in a procedure or corrections, which can be assessed only once a procedure has finished~\cite{ding2023every, ashutosh2023video}
\AF{(this last statement is maybe not 100\% accurate - in some sense our online method also relies on detecting ordering mistakes online)}
, limiting their applicability in real-life scenarios.
At the same time, the spectrum of possible mistakes is indefinitely large, and considering only a part is inadequate.
Given this, the detection of errors should consider their {\it open-set} nature, meaning they are not limited to specific types of errors, and be {\it online} \footnote{Online stands for processing based on causal information and yielding estimates at each frame based on previous frames. This differs from real-time, where specific computational constraints are set as well as required frame rates.}, which means identifying errors as they occur, as waiting until after the procedure is completed is largely ineffective.
% In light of this, mistake detection should consider the {\it open-set'ness} of errors, i.e., not being constrained on specific types of errors, and 
% \AF{aim to make predictions} 
% aim to make predictions {\it online}, i.e., errors are detected as they happen, as detecting them after the procedure has been completed is mostly fruitless. 
% \LS{Possible rephrasing: Given this, the detection of errors should consider their {\it open-set} nature, meaning they are not limited to specific types of errors, and be {\it online} \footnote{Online stands for processing based on causal information and yielding estimates at each frame based on previous frames. This differs from real-time, where specific computational constraints are set as well as required frame rates.}, which means identifying errors as they occur, as waiting until after the procedure is completed is largely ineffective.} 
% \AF{I like the raphrasing.} 
\AF{Not sure I'd stress that offline is largely ineffective - I guess it depends on the application. Imagine a system to assess the quality of production. In that case, offline makes sense, we can still flag mistakes in offline videos to mark the ones which represent a bad execution for review. I believe that online is much more interesting and practical, but maybe we can soften these statements here and there?} 
Despite the practical applications in which online mistake detections would assist, its investigation has been so far limited, with no previous works or benchmarks currently available, which hampers equitable and consistent comparisons.
% Moreover, the absence of a standardized benchmark exacerbates the issue, as it hampers fair and consistent comparisons across the spectrum of newly proposed methods. 
% \LS{Possible rephrasing: Furthermore, the lack of a standardized benchmark compounds the problem by impeding equitable and consistent comparisons. } 
% \AF{Possible alternative rephrasing: Despite the practical applications in which online mistake detections would assist, its investigation has been so far limited, with no previous works or benchmark currently available, which impedes equitable and consistent comparisons.} 
This recognized gap accentuates the need for a novel approach that not only addresses these limitations but also paves the way for more integrative and universally applicable 
% \AF{online?} 
online mistake 
% \AF{mistake rather than error?} 
detection systems.

Inspired by these challenges, this paper proposes a novel approach for detecting errors in PRocedural EGOcentric videos in an online fashion, which we dubbed PREGO. Our methodology hinges on deriving insights exclusively from flawlessly executed procedures, thereby enabling the online identification of errors when an operator's actions diverge from the expected sequence of events as predicted by our network. With this formalization, our proposed method is not constrained to a specific type of mistake, as it can detect any critical deviation from the correct execution of a procedure, labeling it as an error. This approach reveals relations with the neighboring field of Anomaly Detection, where often One-Class Classification (OCC) frameworks are employed to take into account the open-set'ness of anomalies. The architecture of the proposed method is dual-branched \AF{Including a conceptual figure here may help the reader}. The first branch, the {\it action-recognition branch}, analyzes frames in a procedural video up to a current time \(t\), aiming to classify the action being undertaken by the operator. This branch capitalizes on a state-of-the-art video-based online action recognition model, the OadTR Encoder module.
% \AL{OadTR is the encoder-decoder transformer for action recognition. I'd say in the implementation details, as in the paper "Weakly supervised ..", that we use the encoder of OadTR} 
\GD{Should we introduce symbolic reasoning here? Or postpone it to dedicate it its paragraph? I go with this second strategy} 
Concurrently, the second branch, the {\it action-anticipation branch}, assesses the sequence of previously predicted actions up to time \(t-1\) to prognosticate the forthcoming action that the operator should perform. An error is detected upon a misalignment between the currently recognized action and the action anticipated by the predictive model, thereby signaling a deviation from the expected procedure.

\GD{This first draft passes too quickly on the Symbolic Reasoning direction; we should be more specific about why it is smart to graft it in our proposal}
In our in-depth exploration of procedural error detection, we analyze the complexities of the action-anticipation branch, which can be configured in several ways. For instance, it may function as a video stream that processes a more extended context than the {\it current branch}, purposefully focusing on forecasting the immediate subsequent action. Nonetheless, this approach could underutilize the fundamental attribute of procedural learning, which is the sequence of actions that sequentially leads to accomplishing a task. In this work, we propose directly taking advantage of this, representing procedures as sequences and their steps as symbols. This implicit representation removes the semantics from the procedural steps and describes procedures as successions of symbols, eliciting models to discover and reproduce patterns to interpret procedures. Acknowledging this, we draw upon the recent advancements in symbolic reasoning and propose integrating a Large Language Model (LLM) such as LLAMA or GPT-4. This LM is contrived not just to recognize but also to anticipate procedural steps by understanding the sequential patterns of action inherent to a procedure. The model employs symbolic reasoning to span a range of potential actions, adopting a zero-shot next-action label prediction. This prediction leverages the context of accurately performed procedures directly within the query prompt without needing further model fine-tuning, thus allowing the model to harness the knowledge embedded in the span of correctly executed tasks. By incorporating this capability, our method enhances its predictive accuracy, advancing the precision of real-time anomaly detection in executing procedural tasks.

To address these challenges, it becomes crucial to conceive a benchmark that not only labels errors but also considers the impact of these errors on the remaining procedure. Ideally, a procedure should be analyzed up to the first error encountered \AF{while we say this, in Table 2 (if I got this correctly), we evaluate MD besides FMD. Are we considering both scenarios then?}, which more accurately reflects real-world applications where errors necessitate an immediate response to prevent further compounding of the issue. Additionally, such a benchmark should be characterized by 'open-set' conditions, where the system must be able to identify errors that have not been previously encountered or explicitly defined. Given these considerations, our work proposes revising the existing Assembly101 and EpicTent benchmarks. This revision aims to establish a more realistic and challenging scenario for procedural error detection by creating a benchmark that is conducive to training and evaluating systems under open-set conditions and that emphasizes the critical nature of early error detection within a procedure. \AF{This part on the benchmark looks a bit verbose to me. Maybe we could rephrase and summarize in a similar way as ``To support the evaluation of PREGO, we carefully define an online mistake detection benchmark based on the Assembly101 and EpicTent benchmarks. While these benchmarks contain mistake annotation, they have been designed for offline detection. Hence, they contain multiple labeled mistakes beyond the first one. Instead, we propose to...''}

Our evaluation of the PREGO method on the Assembly-101 and EpicTents datasets, which feature natural, non-scripted, and goal-driven procedural egocentric videos, has yielded promising results. By leveraging the advanced symbolic reasoning capabilities of LLMs, PREGO takes strides toward accurate mistake detection.
\GD{old: PREGO effectively discerns errors} \AF{(maybe ``effectively discerns errors'' is a bit overselling, considering that we just said that results are ``promising''?}. It does so by cross-referencing the real-time analyses from an action recognizer with forecasts from a second module, which relies on data from correctly executed procedures of the same task. This comparison between recognized actions and predicted continuations establishes PREGO as a foundational advance in procedural error detection, laying the groundwork for developing even more adept and finely-tuned methodologies.

\input{Tables/comparison_with_sota}
\input{Tables/video-based}
\input{Tables/LLM}

==> sec/Backup/1_intro_2023-11-12.tex <==
\section{Introduction} \label{sec:intro}
% \TD{Sketch of intro
% \begin{itemize}
%     \item using bullets
%     \item This shows the flow of the main argument for problem motivation, what’s missing in related work, and the claimed novelty
% \end{itemize}}


% \FG{The previous bullet list is saved in the backup folder file. I've iterated on the existing valid one, altered the numbers a bit. In general, refer to paragraphs, we'll need those too.}\\
% \GD{Egocentric view is not stressed enough; the connection with our work is in the use-case: a worker wearing an AR device while working gets recommendations and corrections in real-time since the AR device online analyzes his actions and movements.} \AL{"real-time" is something that we should avoid, since the processing is not fast enough for a real time application. I'd remove the references to real-time}
\AL{I think we're giving a lot of space to state we're online and open set. We need to let the reviewer understand why using LLM for symbolic reasoning is the choice. The potential LLM has is huge. We're trying to let it solve hard tasks like ours. }
Procedure learning from the Egocentric point of view is garnering \FG{"attracting". I have never read "garnering" in a paper, it's not necessarily inappropriate, just to say: be sure it's not an odd literal translation from Italian} considerable interest due to the advancements in Robotics and Augmented Reality (AR) 
% Virtual Reality (VR) 
technologies. 
These innovations are not only pivotal for enhancing procedural knowledge and skill acquisition but also play a crucial role in streamlining \FG{maybe add here: "online"\footnote{Most workflows can be aided by \emph{online} monitoring algorithms, which provide feedback to the operator in due course, but may lag due to processing or connectivity delays. We distinguish online from real-time, whereby the second has strict requirements of instantaneous response at all times.}, including the footnote next to online, to clarify online vs real-time} workflow efficiencies\FG{remove "in real-time applications", we do not deal with real-time} in real-time applications.
For instance, AR devices can aid human operators by \FG{providing feedback on the accuracy of their performed tasks and enabling corrective actions in due course} providing instantaneous feedback on the accuracy of their performed tasks, thereby enabling immediate corrective actions.
Recent works have yielded a multitude of datasets~\cite{epicTent,IndustReal,sener2022assembly101,HoloAssist2023,ghoddoosian2022weakly,ding2023every,coin,ikea,IndustReal,cross_task,proceL_2019,howto100m_2019_miech,ragusa2023enigma51} and methodologies aimed at advancing procedure learning~\cite{POC_2022,ghoddoosian2022weakly,OadTR,zhong_2023,epicTent,coin} and error detection~\cite{HoloAssist2023,ding2023every,IndustReal}, particularly within industrial environments.
\FG{from here until the end of the paragraph, there is a duplication of text of the second paragraph. Merge the text, here (if not exceeding max 20 lines) or in the next standalone paragraph. Topic to discuss: 1) online and open-set are needed for real-world applications; 2) no algorithm exists which is online and open-set at the moment} Despite these advancements, 
% \FG{here a stronger criticism of sota: "Despite these advancements, none of the current techniques is applicable in real-world applications, since none of them considers mistakes as open-set recognition problems while also being online, so casually reasoning on the performed procedure} 
% current literature reveals a lack of frameworks that detect errors in procedural egocentric videos for industry applications in an online, open-set, and one-class fashion.
current techniques are unsuitable for real-world applications since they do not treat mistake detection as an open-set recognition problem and do not consider the causality of the problem, i.e., mistakes have to be detected online, considering only the steps before the error occurs.
Indeed, as represented in Table \ref{tab:mistake_methods}, existing approaches typically focus on specific procedural mistakes, e.g., detecting the wrong order of steps or finding missed steps in a procedure, which can often be assessed only once the procedure has finished~\cite{ding2023every, Ghoddoosian_2023_ICCV} 
% \AL{why ref \cite{ashutosh2023video} here? It isn't about mistake detection. I've added ref \cite{Ghoddoosian_2023_ICCV}, which is for online wrong sequence detection (what @antonino is saying in the next comment.}
% \AF{(this last statement is maybe not 100\% accurate - in some sense our online method also relies on detecting ordering mistakes online)}
, limiting their applicability in real-life scenarios.
% \AL{Possible rewording from here:} Indeed, existing methods \TODO{point to table 1?} mainly address procedural errors, such as incorrect sequencing or corrective actions, in a supervised and close-set setting ~\cite{ding2023every, Ghoddoosian_2023_ICCV}. However, this restricts their generalizability to scenarios where diverse and unforeseen mistakes may occur, or it's not practical to label or produce erroneous videos. \AL{to here.}
% \FG{merge this paragraph or its rewording above to the first paragraph. I'd start the second paragraph with our arguments.}

\FG{See my note above on the repetition} We argue that {\it online} and {\it open-set} aspects are crucial when implementing egocentric models for real-world applications. The {\it online} factor signifies continuous, causal processing, vital for dynamic decision-making and immediate response. The {\it open-set} trait describes the mistakes as anything unexpected, as a procedural mistake is anything that hinders the procedure from being completed successfully.
% \FG{I'd open the second paragraph with a clear top-down statement of the important ingredients we argue for, to clarify both of them are essential, in certain applications. Eg "We argue that online and open-set are two essential attributes when applying egocentric models to .. applications. The first stands for causal processing..[other arguments].. The second, open-set, enables consider mistakes as anything unexpected, as a procedural mistake is anything which hinders the procedure from completing successfully, without the need to deploy correction procedures.}
% At the same time, the spectrum of possible mistakes is indefinitely large and, most of the time, unknown in advance. Hence, considering only a part is inadequate.
% Considering this, the detection of errors should consider their {\it open-set} nature, meaning they are not limited \AL{constrained} to specific types of errors, \AL{should we add here that we want it also one-class?} and be {\it online} \footnote{Online stands for processing based on causal information and yielding estimates at each frame based on previous frames. This differs from real-time, where specific computational constraints are set as well as required frame rates.}, which means identifying errors as they occur, as waiting until after the procedure is completed is largely ineffective.
% In light of this, mistake detection should consider the {\it open-set'ness} of errors, i.e., not being constrained on specific types of errors, and 
% \AF{aim to make predictions} 
% aim to make predictions {\it online}, i.e., errors are detected as they happen, as detecting them after the procedure has been completed is mostly fruitless. 
% \LS{Possible rephrasing: Given this, the detection of errors should consider their {\it open-set} nature, meaning they are not limited to specific types of errors, and be {\it online} \footnote{Online stands for processing based on causal information and yielding estimates at each frame based on previous frames. This differs from real-time, where specific computational constraints are set as well as required frame rates.}, which means identifying errors as they occur, as waiting until after the procedure is completed is largely ineffective.} 
% \AF{I like the raphrasing.} 
% \AF{Not sure I'd stress that offline is largely ineffective - I guess it depends on the application. Imagine a system to assess the quality of production. In that case, offline makes sense, we can still flag mistakes in offline videos to mark the ones which represent a bad execution for review. I believe that online is much more interesting and practical, but maybe we can soften these statements here and there?}
% From here
Despite the practical applications in which online and open-set mistake detections would assist, its investigation has been so far limited, with no previous works or benchmarks currently available, which hampers equitable and consistent comparisons. 
% \AL{we cannot say that no one has done it online if we have two ticks in table 1. No one has done it in one-class and online.}
% Moreover, the absence of a standardized benchmark exacerbates the issue, as it hampers fair and consistent comparisons across the spectrum of newly proposed methods. 
% \LS{Possible rephrasing: Furthermore, the lack of a standardized benchmark compounds the problem by impeding equitable and consistent comparisons. } 
% \AF{Possible alternative rephrasing: Despite the practical applications in which online mistake detections would assist, its investigation has been so far limited, with no previous works or benchmark currently available, which impedes equitable and consistent comparisons.} 
This gap spotlights the need for a novel approach that addresses these limitations and paves the way for more integrative and universally applicable 
online mistake detection systems.

% Inspired by these challenges\FG{inspired by challenges?? maybe to tackle these challenges. But I'd have a positive start of this third paragraph, eg "Here we propose the first model to detect PRocedural errors in EGOcentric videos (PREGO), which is both online, thus causal, and open-set, training a one-class classifier on correct procedures just."}, this paper proposes a novel approach for detecting errors in PRocedural EGOcentric videos in an online \AL{and open-set/one-class} fashion, which we dubbed \emph{PREGO}.
In this work, we propose the first model to detect PRocedural errors in EGOcentric videos (PREGO), which is both online, thus causal, and open-set, not limited to specific types of procedural mistakes. The online attribute is achieved by analyzing input videos sequentially up to a given frame \(t\), ensuring that no future actions influence the current step recognition. \FG{remove this sentence, repetition, and real-time not applicable} This approach is essential for maintaining the causality of the process, as it prevents foresight of future steps, enabling the model to react to events as they unfold in real-time. On the other hand, the open-set is performed by exclusively exposing PREGO to correct procedural sequences when anticipating the next steps. \FG{remove this sentence, repetition} This design choice compels the model to identify errors by detecting deviations from correct similar example sequences. Any step within a procedure that significantly diverges from the established correct patterns is deemed an error, allowing PREGO to recognize a wide range of procedural mistakes without being confined to a restricted set of predefined errors. \FG{remove this sentence, repetition}This novel approach enables PREGO to adaptively identify procedural errors in various real-world settings, making it an effective tool in egocentric video analysis.
% \FG{this sentence is a repetition, it's explained in the second paragraph}Our methodology hinges on deriving insights exclusively from flawlessly executed procedures, thereby enabling the online identification of errors when an operator's actions diverge from the expected sequence of events as predicted by our network.
% With this formalization, \AL{I'd remove "With this formalization"} \FG{this sentence is a repetition, it's explained in the second paragraph} our proposed method is not constrained to a specific type of mistake, as it can detect any critical deviation from the correct execution of a procedure, labeling it as an error.
\FG{re-reading this sentence, I'd remove the reference to VOD here, and just leave it in the related work. In general, remove this sentence altogether, and merge OCC above where learning on correct procedures just is named} This approach reveals relations with the One-Class Classification (OCC) framework typically employed in the neighboring field of Video Anomaly Detection \TODO{ref?} to take into account the open-setness of anomalies \FG{ok to mention, but this implies that we need to analyze the relations, what techniques can be taken from that field}.


PREGO's architecture is dual-branched, as depicted in Fig.~\ref{fig:framework_pic}.
% \AF{Including a conceptual figure here may help the reader}.
The first branch, the {\it step-recognition branch}, analyzes frames in a procedural video up to a current time \(t\), aiming to classify the action being undertaken by the operator.
This branch capitalizes on a state-of-the-art video-based online action recognition model, the OadTR~\cite{OadTR} Encoder module. 
% \AL{it is not totally clear the connection from frames to label space of the LLMs.}
% \AL{OadTR is the encoder-decoder transformer for action recognition. I'd say in the implementation details, as in the paper "Weakly supervised ..", that we use the encoder of OadTR} 
% \GD{Should we introduce symbolic reasoning here? Or postpone it to dedicate it its paragraph? I go with this second strategy} 
% \ED{I'd anticipate it here and then deepen it later}
Concurrently, the second branch is in charge of \emph{step-anticipation}: an LLM~\cite{touvron2023llama} assesses the sequence of previously predicted actions up to time $t-1$, and predicts the $t$-th action in a zero-shot manner.
% Concurrently, the second branch, the {\it action-anticipation branch}, assesses the sequence of previously predicted actions up to time \(t-1\) to prognosticate the forthcoming action that the operator should perform. 
An error is detected upon a misalignment between the currently recognized action and the one anticipated, 
% by the predictive model
thereby signaling a deviation from the expected procedure.
% \FG{In my view, it's ok to have the description of the two branches here, and to mention that video recognition leverages a sota technique, oadtr.}

% \FG{Start and dedicate this fourth paragraph to symbolic reasoning for action anticipation/next action prediction. Eg "we propose to perform next action prediction, for the first time, by means of a foundational LLM, educated to perform zero-shot symbolic reasoning by the use of context.." And cite the best papers in cvpr'23 and iccv'23}
For the first time, we propose to perform next action prediction using a pre-trained Large Language Model (LLM) for zero-shot symbolic reasoning through contextual analysis. This approach marks a significant shift from previous literature in procedural learning, suggesting repositioning from semantic-based expressions of procedures to an implicit representation, where only patterns of symbols have to be recognized and predicted. By representing procedures as sequences and their steps as symbols, we let the predictor focus on the patterns that characterize the correct procedures. \FG{remove this sentence, repetition} This strategy enables our models to discern and replicate patterns essential for interpreting procedures.
Leveraging the advancements in symbolic reasoning~\cite{surismenon2023vipergpt,Gupta_2023_visualprog,generalpatternmachines2023}, we integrate an LLM~\cite{touvron2023llama} into our framework. \FG{from here}This module is in charge of predicting procedural steps by capturing the sequential patterns intrinsic to a task. It employs symbolic reasoning to consider a range of possible actions, executing in-context zero-shot next-symbol prediction. Indeed, this approach exploits the correctly performed procedures as examples within the query prompt itself, eliminating the need for additional model fine-tuning. By incorporating this capability, our method enhances its predictive accuracy, advancing the precision of online mistake detection, as our comprehensive experiments maintain.\FG{to here, it's a repetition of the first part of this paragraph. Merge/remove one of the two. However, in this paragraph, we need to add a specific reference to: 1) multiple plausible ways of accomplishing an action; 2) representation learning of action dependencies in the procedures.}

%%%%%%%%%%%%% fourth par %%%%%%%%%
% \GD{This first draft passes too quickly on the Symbolic Reasoning direction; we should be more specific about why it is smart to graft it in our proposal}
% In our in-depth exploration of procedural error detection, we analyze the complexities of the action-anticipation branch, which can be configured in several ways. 
% For instance, it may function as a video stream that processes a more extended context than the {\it current branch}, purposefully focusing on forecasting the subsequent action. Nonetheless, this approach could not fully leverage the essential attribute of procedural learning, which is the sequence of actions that sequentially leads to accomplishing a task. 
% In this work, we propose directly taking advantage of this, representing procedures as sequences and their steps as symbols. 
% This implicit representation removes the semantics from the procedural steps and describes procedures as successions of symbols, eliciting models to discover and reproduce patterns to interpret procedures. 
% Acknowledging this, we draw upon the recent advancements in symbolic reasoning and propose integrating a Large Language Model (LLM) \TODO{add ref} such as LLAMA-2 or GPT-4\ED{I would avoid mentioning GPT-4, I'd speak of LLMs in general and only name the ones we texted (LLAMA-2 and GPT-3.5}. 
% This LM is contrived not just to recognize but also to anticipate procedural steps by understanding the sequential patterns of action inherent to a procedure. 
% The model employs symbolic reasoning to span a range of potential actions, adopting a zero-shot next-action label prediction. 
% This prediction leverages the context of correctly performed procedures directly within the query prompt without needing further model fine-tuning, thus allowing the model to harness the knowledge embedded in the span of correctly executed tasks.
% By incorporating this capability, our method enhances its predictive accuracy, advancing the precision of online
% % \AL{I'd avoid the use of real-time} 
% anomaly detection in executing procedural tasks.
%%%%%%%%%%%%%%%%%%%%

% To address these challenges, it becomes crucial to conceive a benchmark that not only labels errors but also considers the impact of these errors on the remaining procedure. 
% Ideally, a procedure should be analyzed up to the first error encountered \AF{while we say this, in Table 2 (if I got this correctly), we evaluate MD besides FMD. Are we considering both scenarios then?}, which more accurately reflects real-world applications where errors necessitate an immediate response to prevent further compounding of the issue. 
% Additionally, such a benchmark should be characterized by 'open-set' conditions, where the system must be able to identify errors that have not been previously encountered or explicitly defined.
% Given these considerations, our work proposes revising the existing Assembly101~\cite{sener2022assembly101} and EpicTent~\cite{epicTent} benchmarks. 
% This revision aims to establish a more realistic and challenging scenario for procedural error detection by creating a benchmark that is conducive to training and evaluating systems under open-set conditions and that emphasizes the critical nature of early error detection within a procedure. 
% \AF{This part on the benchmark looks a bit verbose to me. Maybe we could rephrase and summarize in a similar way as ``To support the evaluation of PREGO, we carefully define an online mistake detection benchmark based on the Assembly101 and EpicTent benchmarks. While these benchmarks contain mistake annotation, they have been designed for offline detection. Hence, they contain multiple labeled mistakes beyond the first one. Instead, we propose to...''}
To support the evaluation of PREGO, we \FG{remove "carefully", all papers are such} carefully \FG{"define" risks being an overstatement. I'd prefer "review the procedural benchmarks of x and y, setting the novel task of online mistake detection" } define an online mistake detection benchmark based on the Assembly101~\cite{sener2022assembly101} and EpicTent~\cite{epicTent} benchmarks. While these benchmarks contain mistake annotations, they have been designed for offline detection. Therefore, they include multiple labeled mistakes beyond the initial error. To adapt these benchmarks for online detection, we propose to focus exclusively on the first mistake in each procedural sequence. This approach aligns with the real-world application of a mistake detector, which aims to detect and address errors as they occur rather than analyzing a complete sequence of multiple errors post-event.
By concentrating on the first mistake, we can more accurately assess PREGO's efficacy and its ability to prevent cascading errors in procedural tasks. This modification also aligns the benchmarks with the practical needs of industries and domains where immediate error detection is crucial for maintaining process integrity and safety. A second modification we operate to the original dataset concerns the splits. Indeed, \cite{sener2022assembly101} exposes a dataset split that allows only supervised mistake detection tasks, with erroneous sequences occurring in the trainset. To enable an OCC framework, we revisit the current split leaving all the mistaken procedures in the test set. This novel benchmark will serve as a more robust testing ground for PREGO and set a new standard for evaluating online procedural error detection models in future research.
\FG{Overall, this section confuses our model choice (OCC) with the benchmark definition (online). I'd suggest reviewing the main concepts here:\\
1) we review the assembly101 and epictents benchmarks to set a new task challenge, online procedural mistake detection\\
2) online procedural mistake detection calls for raising an error flag in due course, as soon as the current initiated action sets a procedure that is not plausible (even in view of multiple plausible pathways)\\
3) so we benchmark videos for online correctness up until the first mistakes (when the machine supposedly provides feedback and suggests corrective procedures)\\
One extra remark might regard the reshuffling of videos:\\
1) correct only videos are best fit in the training set, to balance the amount of correct vs incorrect videos;\\
2) training/val/test videos should contain the same procedures in similar distribution, we do not want novel actions at test, this is not a novel action classification, we assume all procedures in all multiple plausible ways are provided at training.\\
OCC is our choice (to deal with openset), do not include this into the benchmarking paragraph. And up to the first error in training is also our choice, and it's only about our llm branch, so do not include reference to his here.}

\FG{This paragraph is all repetition, remove it. Just add to the previous paragraph a single sentence, eg "The novel online procedural mistakes detection benchmark tasks in assembly101 and epictents are challenging but the results of PREGO are encouraging"}Our evaluation of the PREGO method on the Assembly-101~\cite{sener2022assembly101} and EpicTent~\cite{epicTent} datasets, which feature natural, non-scripted, and goal-driven procedural egocentric videos, has yielded promising results. By leveraging the advanced symbolic reasoning capabilities of LLMs, PREGO takes strides toward accurate mistake detection.
% \GD{old: PREGO effectively discerns errors} 
% \AF{(maybe ``effectively discerns errors'' is a bit overselling, considering that we just said that results are ``promising''?}. 
It does so by cross-referencing the online analyses from an action recognizer with forecasts from a second module, which relies on data from correctly executed procedures of the same task. This comparison between recognized actions and predicted continuations establishes PREGO as a foundational advance in procedural error detection, laying the groundwork for developing even more adept and finely-tuned methodologies.

\input{Tables/comparison_with_sota}


==> sec/Backup/1_intro_2023-11-16.tex <==
\section{Introduction} \label{sec:intro}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Images/concept.pdf}%{Images/prego_placeholder.pdf}
    \caption{\AF{Procedural activities require steps to be performed following a correct ordering. We propose to detect procedural mistakes online by assessing inconsistencies between the keystep executed at time $t$ and a prediction made by an anticipation model observing previous keysteps at previous timestamps.} \AF{We need some sort of conceptual figure. I put a placeholder just to get the conversation started. Feel free to remove/edit drastically - the pptx in the ``Images'' folder.}\FG{Very good first draft. Maybe it's useful to be more accurate about our proposed technique: the video recognizer ingests frames and outputs labels (up to t), the symbolic reasoner ingests labels (up to t-1) and predicts that at t, which is then compared.    I like the idea to cartoonize the models. Some ideas might be: we may need two models/robots; the video recognizers should have eyes/show that they leverage images; the symbolic reasoners should somehow depict the llm-like internal monologue of the robot (la nuvoletta che rappresenta il pensiero nei fumetti, come c'e' ora).}\AL{I was thinking that we can add a cartoonized LLAMA for the LLM part.}
    }
    \label{fig:conceptual}
\end{figure}


Procedure learning from the Egocentric point of view is attracting considerable interest due to the advancements in Robotics and Augmented Reality (AR) technologies. 
These innovations are pivotal for enhancing procedural knowledge and skill acquisition and play a crucial role in streamlining online\footnote{Most workflows can be aided by \emph{online} monitoring algorithms, which provide feedback to the operator in due course. However, they may lag due to processing or connectivity delays. We distinguish online from real-time, whereby the second has strict requirements of instantaneous response.} workflow efficiencies.
For instance, AR devices can aid human operators by providing feedback on the accuracy of their performed tasks and enabling corrective actions in due course.
Recent works have yielded a multitude of datasets~\cite{epicTent,IndustReal,sener2022assembly101,HoloAssist2023,ghoddoosian2022weakly,ding2023every,coin,ikea,IndustReal,cross_task,proceL_2019,howto100m_2019_miech,ragusa2023enigma51} and methodologies aimed at advancing procedure learning~\cite{POC_2022,ghoddoosian2022weakly,OadTR,zhong_2023,epicTent,coin} and error detection~\cite{HoloAssist2023,ding2023every,IndustReal}, particularly within industrial environments.
Despite these advancements, existing methods prove impractical for real-world scenarios as they do not cast mistake detection as an {\it online} and {\it open-set} problem.
The {\it online} factor signifies continuous, causal processing, vital for dynamic decision-making and immediate response. The {\it open-set} trait describes the mistakes as anything unexpected, as a procedural mistake is anything that hinders the procedure from being completed successfully.
As illustrated in Table~\ref{tab:mistake_methods}, prevailing methodologies commonly concentrate on isolated procedural errors, such as identifying missteps in the order or detecting omitted steps within a procedure. However, these assessments are often viable only once the entire procedure has concluded~\cite{ding2023every, Ghoddoosian_2023_ICCV}, constraining their relevance in real-world situations.
This gap spotlights the need for a novel approach that addresses these limitations and paves the way for more integrative and universally applicable online mistake detection systems.
\FG{This paragraph needs to be shortened. I'd recommend reordering to streamline: reference to methodologies (list of citations); reference to table 1; state that there are a few open-set techniques and a few online techniques, but no research has addressed both, which is important for real-world applications.}
% \FG{from here until the end of the paragraph, there is a duplication of text of the second paragraph. Merge the text, here (if not exceeding max 20 lines) or in the next standalone paragraph. Topic to discuss: 1) online and open-set are needed for real-world applications; 2) no algorithm exists which is online and open-set at the moment} Despite these advancements, current techniques are unsuitable for real-world applications since they do not treat mistake detection as an open-set recognition problem and do not consider the causality of the problem, i.e., mistakes have to be detected online, considering only the steps before the error occurs.
% Indeed, as represented in Table \ref{tab:mistake_methods}, existing approaches typically focus on specific procedural mistakes, e.g., detecting the wrong order of steps or finding missed steps in a procedure, which can often be assessed only once the procedure has finished~\cite{ding2023every, Ghoddoosian_2023_ICCV}, limiting their applicability in real-life scenarios.
% \FG{See my note above on the repetition} We argue that {\it online} and {\it open-set} aspects are crucial when implementing egocentric models for real-world applications. The {\it online} factor signifies continuous, causal processing, vital for dynamic decision-making and immediate response. The {\it open-set} trait describes the mistakes as anything unexpected, as a procedural mistake is anything that hinders the procedure from being completed successfully.
% Despite the practical applications in which online and open-set mistake detections would assist, its investigation has been so far limited, with no previous works or benchmarks currently available, which hampers equitable and consistent comparisons. 
% This gap spotlights the need for a novel approach that addresses these limitations and paves the way for more integrative and universally applicable 
% online mistake detection systems.

In this work, we propose the first model to detect PRocedural errors in EGOcentric videos (PREGO), which is both online, thus causal, and open-set, not limited to specific procedural mistakes. The online attribute is achieved by analyzing input videos sequentially up to a given frame \(t\), ensuring that no future actions influence the current step recognition. 
On the other hand, the open-set is performed by exclusively exposing PREGO to correct procedural sequences when anticipating the next steps following the One-Class Classification (OCC) paradigm. Any step within a procedure that significantly diverges from the established correct patterns is deemed an error, allowing PREGO to recognize a wide range of procedural mistakes without being confined to a restricted set of predefined errors. 

% \FG{re-reading this sentence, I'd remove the reference to VOD here, and just leave it in the related work. In general, remove this sentence altogether, and merge OCC above where learning on correct procedures just is named} This approach reveals relations with the One-Class Classification (OCC) framework typically employed in the neighboring field of Video Anomaly Detection \TODO{ref?} to take into account the open-setness of anomalies \FG{ok to mention, but this implies that we need to analyze the relations, what techniques can be taken from that field}.


PREGO's architecture is dual-branched, as depicted in Fig.~\ref{fig:framework_pic}.
The first branch, the {\it step-recognition branch}, analyzes frames in a procedural video up to a current time \(t\), aiming to classify the action being undertaken by the operator.
This branch capitalizes on a state-of-the-art video-based online action recognition model, the OadTR~\cite{OadTR} Encoder module. 
Concurrently, the second branch is in charge of \emph{step-anticipation}: an LLM~\cite{touvron2023llama} assesses the sequence of previously predicted actions up to time $t-1$, and predicts the $t$-th action in a zero-shot manner.
An error is detected upon a misalignment between the currently recognized action and the one anticipated, thereby signaling a deviation from the expected procedure.

For the first time, we propose to perform next action prediction using a pre-trained Large Language Model (LLM)~\cite{touvron2023llama} for zero-shot symbolic reasoning through contextual analysis~\cite{surismenon2023vipergpt,Gupta_2023_visualprog,generalpatternmachines2023}. 
Utilizing correctly executed procedures as instances in the query prompt obviates the necessity for additional model fine-tuning. 
This approach marks a significant shift from previous literature in procedural learning \FG{what shift?? saying "a significant shift" requires explaining. I'd probably rephrase: "Our proposed approach is an abstraction from the video content. Using labels allows for longer-term reasoning, as a label summarizes several frames. Also, this approach is an alternative to the carefully constructed graphs of action inter-pedendencies [ref]. We demonstrate that symbolic reasoning subsumes understanding long procedures and the action inter-dependencies}, suggesting repositioning from semantic-based expressions of procedures to an implicit representation, where only patterns of symbols have to be recognized and predicted. By representing procedures as sequences and their steps as symbols, we let the predictor focus on the patterns that characterize the correct procedures. 
\FG{However, in this paragraph, we need to add a specific reference to: 1) multiple plausible ways of accomplishing an action; 2) representation learning of action dependencies in the procedures.}\GD{I didn't get this second bullet}\FG{See the proposed rephrasing}

% For the first time, we propose to perform next action prediction using a pre-trained Large Language Model (LLM) for zero-shot symbolic reasoning through contextual analysis. This approach marks a significant shift from previous literature in procedural learning, suggesting repositioning from semantic-based expressions of procedures to an implicit representation, where only patterns of symbols have to be recognized and predicted. By representing procedures as sequences and their steps as symbols, we let the predictor focus on the patterns that characterize the correct procedures. 
% Leveraging the advancements in symbolic reasoning~\cite{surismenon2023vipergpt,Gupta_2023_visualprog,generalpatternmachines2023}, we integrate an LLM~\cite{touvron2023llama} into our framework. \FG{from here}This module is in charge of predicting procedural steps by capturing the sequential patterns intrinsic to a task. It employs symbolic reasoning to consider a range of possible actions, executing in-context zero-shot next-symbol prediction. Indeed, this approach exploits the correctly performed procedures as examples within the query prompt itself, eliminating the need for additional model fine-tuning. By incorporating this capability, our method enhances its predictive accuracy, advancing the precision of online mistake detection, as our comprehensive experiments maintain.\FG{to here, it's a repetition of the first part of this paragraph. Merge/remove one of the two. However, in this paragraph, we need to add a specific reference to: 1) multiple plausible ways of accomplishing an action; 2) representation learning of action dependencies in the procedures.}

%%%%%%%%%%%%% fourth par %%%%%%%%%
To support the evaluation of PREGO, we review the procedural benchmarks of Assembly101~\cite{sener2022assembly101}  and EpicTent~\cite{epicTent}, setting the novel task of online procedural
% \GF{procedural} 
mistake detection.
\FG{Possible rephrasing (see my note below): "In the reviewed online benchmarks, which we dub Assembly101-O and EpicTent-O, the model is tasked with asserting the occurrence of the procedural mistake as soon as it happens. While multiple procedures may be plausible, Assembly101-O and EpicTent-O mark as mistake the first action, after which the procedure cannot successfully complete.", or something similar. Then REMOVE FROM HERE:}
While original benchmarks contain mistake annotations, they have been designed for offline detection. 
Therefore, they include multiple labeled mistakes beyond the first error. 
To adapt these online detection benchmarks, we propose focusing exclusively on the first mistake in each procedural sequence. 
This approach aligns with the real-world application of a mistake detector, which aims to detect and address errors as they occur rather than analyzing a complete sequence of multiple errors post-event.
By concentrating on the first mistake, we can more accurately assess PREGO's efficacy and ability to prevent cascading errors in procedural tasks. 
This modification also aligns the benchmarks with the practical needs of industries and domains where immediate error detection is crucial for maintaining process integrity and safety.
This novel benchmark will serve as a more robust testing ground for PREGO and set a new standard for evaluating online procedural error detection models in future research.\FG{TO HERE.}
Moreover, despite a challenging task, PREGO's results are particularly promising, underscoring its effectiveness and potential in advancing the field.
\FG{I find these statements a bit tricky. Effectively the current datasets have corrective procedures, which we exclude. Saying that we exclude corrective procedures is not a bonus for us. I mean: we do it because it'd be difficult to also learn corrections, but it may be seen as our limitation, which should not have influenced our data preparation. My suggestion would be to stay away from statements on the detriments of multiple mistakes in a video. So take a positive writing perspective, proposing our review and motivating it.
Effectively, our decision to consider the first mistake is a limitation, which we should acknowledge in a section for "limitations and future work", just before the conclusions.}

% A second modification we operate to the original dataset concerns the splits. Indeed, \cite{sener2022assembly101} exposes a dataset split that allows only supervised mistake detection tasks, with erroneous sequences occurring in the trainset. To enable an OCC framework, we revisit the current split leaving all the mistaken procedures in the test set. 
% \FG{Overall, this section confuses our model choice (OCC) with the benchmark definition (online). I'd suggest reviewing the main concepts here:\\
% 1) we review the assembly101 and epictents benchmarks to set a new task challenge, online procedural mistake detection\\
% 2) online procedural mistake detection calls for raising an error flag in due course, as soon as the current initiated action sets a procedure that is not plausible (even in view of multiple plausible pathways)\\
% 3) so we benchmark videos for online correctness up until the first mistakes (when the machine supposedly provides feedback and suggests corrective procedures)\\
% \FG{One extra remark might regard the reshuffling of videos:\\
% 1) correct only videos are best fit in the training set, to balance the amount of correct vs incorrect videos;\\
% 2) training/val/test videos should contain the same procedures in similar distribution, we do not want novel actions at test, this is not a novel action classification, we assume all procedures in all multiple plausible ways are provided at training.} 
% \AL{I vari esperimenti ci hanno alla fine portato a dover considerare solo ATTACH-THIS (senza that quindi). Abbiamo quindi che train = all normal procedures, test = procedures with mistakes. In questo modo sono presenti solo 86 azioni in tutto (invece di 297). mAP è passata al 14\% in questo caso, negli altri esperimenti invece siamo arrivati al massimo a 7\%. } \\
% OCC is our choice (to deal with openset), do not include this into the benchmarking paragraph. And up to the first error in training is also our choice, and it's only about our llm branch, so do not include reference to his here.}

% \FG{This paragraph is all repetition, remove it. Just add to the previous paragraph a single sentence, eg "The novel online procedural mistakes detection benchmark tasks in assembly101 and epictents are challenging but the results of PREGO are encouraging"}Our evaluation of the PREGO method on the Assembly-101~\cite{sener2022assembly101} and EpicTent~\cite{epicTent} datasets, which feature natural, non-scripted, and goal-driven procedural egocentric videos, has yielded promising results. By leveraging the advanced symbolic reasoning capabilities of LLMs, PREGO takes strides toward accurate mistake detection.

% It does so by cross-referencing the online analyses from an action recognizer with forecasts from a second module, which relies on data from correctly executed procedures of the same task. This comparison between recognized actions and predicted continuations establishes PREGO as a foundational advance in procedural error detection, laying the groundwork for developing even more adept and finely-tuned methodologies.

\FG{Add a bulleted list of Contributions: "We summarize our contributions as follows:"..}

\input{Tables/comparison_with_sota}


==> sec/Backup/1_intro_2024-03-07-.tex <==
\section{Introduction} \label{sec:intro}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Images/teaser.pdf}%{Images/prego_placeholder.pdf}
    \caption{
    % \AF{
    PREGO is based on two main components: The recognition module (top) processes the input video in an online fashion and predicts actions observed at each timestep; the anticipation module (bottom) reasons symbolically via a Large Language Model to predict the future action based on past action history and a short context of previous action sequences \AL{to be better described the context part}. Mistakes are identified when the currently detected action \AL{by the step recognition method} differs from the one anticipated from past action history \AL{by the step anticipation module} (right).}
    % } 
    % \AF{Maybe we could add the ``LLM'' text under the lama icon?} \FG{the recognition module needs to also have an arrow from the current frame. It currently seems omitted, which may give a wrong idea. So it should not be grayed, and there should be an arrow. Question relating to the recognizer: why don't you make the corresponding top arrows (currently black) of the same color as their corresponding bottom arrows (orange, green, blue)? it's not visually easy to follow and discern black arrows.}
    % \FG{Question: shall we pictorially show someone wearing glasses? see the assembly101 dataset}
    % \AF{Maybe that could replace the robot?}}
    \label{fig:conceptual}
\end{figure}

% Comment on teaser:
% \GF{GMF: In this figure seems that both models consider video until time t-1. the robot model has to consider until t. There shouls be not a ? but the cell with color blue at time t.}\GD{right, thanks!} \AF{Procedural activities require steps to be performed following a correct ordering. We propose to detect procedural mistakes online by assessing inconsistencies between the keystep executed at time $t$ and a prediction made by an anticipation model observing previous keysteps at previous timestamps.} \AF{We need some sort of conceptual figure. I put a placeholder just to get the conversation started. Feel free to remove/edit drastically - the pptx in the ``Images'' folder.}\FG{Very good first draft. Maybe it's useful to be more accurate about our proposed technique: the video recognizer ingests frames and outputs labels (up to t), the symbolic reasoner ingests labels (up to t-1) and predicts that at t, which is then compared.    I like the idea to cartoonize the models. Some ideas might be: we may need two models/robots; the video recognizers should have eyes/show that they leverage images; the symbolic reasoners should somehow depict the llm-like internal monologue of the robot (la nuvoletta che rappresenta il pensiero nei fumetti, come c'e' ora).}\AL{I was thinking that we can add a cartoonized LLAMA for the LLM part.}

Egocentric procedure learning is gaining attention due to advancements in Robotics and Augmented Reality (AR) technologies. These technologies are pivotal in improving online\footnote{Most workflows can be aided by \emph{online} monitoring algorithms, which provide feedback to the operator in due course. However, they may lag due to processing or connectivity delays. We distinguish online from real-time, whereby the second has strict requirements of instantaneous response.} monitoring by providing timely feedback to the operator.
Recent works have produced numerous datasets~\cite{epicTent,IndustReal,sener2022assembly101,HoloAssist2023,Ghoddoosian_2023_ICCV,ding2023every,coin,ikea,IndustReal,cross_task,proceL_2019,howto100m_2019_miech,ragusa2023enigma51}, methodologies aimed at advancing procedure learning~\cite{POC_2022,Ghoddoosian_2023_ICCV,OadTR,zhong_2023,epicTent,coin} and error detection models~\cite{HoloAssist2023,ding2023every,IndustReal}.
% , particularly within industrial environments.
Despite these advancements, as outlined in Table~\ref{tab:mistake_methods}, prevalent methodologies typically focus on isolated procedural errors, like pinpointing missteps in sequence or identifying omitted steps within a procedure. They are unsuitable for situations requiring dynamic decision-making, specifically in an {\it online} context, or in cases where mistakes can be unexpected—hence, characterized as an {\it open-set}.


% \LS{You can find the previous version commented below.}
% Despite these advancements, current methods are unsuitable for real-world scenarios because they do not frame mistake detection as an {\it online} and {\it open-set} problem.
% The {\it online} factor signifies continuous, causal processing, vital for dynamic decision-making and immediate response. The {\it open-set} trait describes the mistakes as anything unexpected, as a procedural mistake is anything that hinders the procedure from being completed successfully. \LS{Possible rephrasing: The {\it open-set} characteristic defines mistakes as anything unexpected, whereas a procedural mistake is anything that obstructs the successful completion of the procedure.}
% As illustrated in Table~\ref{tab:mistake_methods}, prevailing methodologies commonly concentrate on isolated procedural errors, such as identifying missteps in the order or detecting omitted steps within a procedure. However, these assessments are often viable only once the entire procedure has concluded~\cite{ding2023every, Ghoddoosian_2023_ICCV}, constraining their relevance in real-world situations.
% This gap spotlights the need for a novel approach that addresses these limitations and paves the way for more integrative and universally applicable online mistake detection systems.
% \FG{This paragraph needs to be shortened. I'd recommend reordering to streamline: reference to methodologies (list of citations); reference to table 1; state that there are a few open-set techniques and a few online techniques, but no research has addressed both, which is important for real-world applications.}
\input{Tables/comparison_with_sota}


In this work, we propose the first model to detect PRocedural errors in EGOcentric videos (PREGO), which is both online, thus causal, and open-set, not limited to specific kinds of procedural mistakes. The online attribute is achieved by analyzing input videos sequentially up to a given frame \(t\), ensuring that no future actions influence the current step recognition. 
On the other hand, the open-set learning is performed by exclusively exposing PREGO to correct procedural sequences 
when predicting mistakes,
%>> OLD VERSION: non abbiamo ancora parlato di anticipation in intro e goal finale è predire mistake
%when anticipating the next steps 
following the One-Class Classification (OCC) paradigm \AL{ref?}. Any step within a procedure that significantly diverges from the
expected
%>> OLD VERSION: established sembra implicare che abbiamo formalmente stabilito cosa è giusto e cosa no
%established 
correct patterns is deemed an error, allowing PREGO to recognize a wide range of procedural mistakes without being confined to a restricted set of predefined errors. 

PREGO's architecture is dual-branched, as depicted in Fig.~\ref{fig:conceptual}.
The first branch, the {\it step-recognition branch}, analyzes frames in a procedural video up to a current time \(t\), aiming to classify the action being undertaken by the operator.
This branch capitalizes \AL{capitalizes?} on a state-of-the-art video-based online step recognition model, the OadTR~\cite{OadTR} Encoder module. 
Concurrently, the second branch is in charge of \emph{step-anticipation}: 
a Large Language Model (LLM)~\cite{touvron2023llama}
%>>OLD VERSION:
%an LLM~\cite{touvron2023llama} 
assesses the sequence of previously predicted actions up to time $t-1$, and predicts the $t$-th action in a zero-shot manner.
An error is detected upon a misalignment between the currently recognized action and the anticipated one,
%>>OLD:
%one anticipated, 
thereby signaling a deviation from the expected procedure.

For the first time, we propose to perform next action prediction using a pre-trained Large Language Model (LLM)~\cite{touvron2023llama} for zero-shot symbolic reasoning through contextual analysis~\cite{surismenon2023vipergpt,gupta2023visual,generalpatternmachines2023}. 
Utilizing correctly executed procedures as instances in the query prompt obviates the necessity for additional model fine-tuning and leverages the pattern-completion abilities of LLMs.
Our proposed approach is an abstraction from the video content. Using labels allows for longer-term reasoning, as a label summarizes several frames. Also, this approach is an alternative to the carefully constructed action inter-dependency graphs~\cite{ashutosh2023video}. We demonstrate that symbolic reasoning subsumes understanding long procedures and the action inter-dependencies, suggesting repositioning from semantic-based expressions of procedures to an implicit representation, where only patterns of symbols have to be recognized and predicted. By representing procedures as sequences and their steps as symbols, we let the predictor focus on the patterns that characterize the correct procedures. 
% This approach marks a significant shift from previous literature in procedural learning \FG{what shift?? saying "a significant shift" requires explaining. I'd probably rephrase: "Our proposed approach is an abstraction from the video content. Using labels allows for longer-term reasoning, as a label summarizes several frames. Also, this approach is an alternative to the carefully constructed graphs of action inter-pedendencies [ref]. We demonstrate that symbolic reasoning subsumes understanding long procedures and the action inter-dependencies}, suggesting repositioning from semantic-based expressions of procedures to an implicit representation, where only patterns of symbols have to be recognized and predicted. By representing procedures as sequences and their steps as symbols, we let the predictor focus on the patterns that characterize the correct procedures. 
% \FG{However, in this paragraph, we need to add a specific reference to: 1) multiple plausible ways of accomplishing an action; 2) representation learning of action dependencies in the procedures.}\GD{I didn't get this second bullet}\FG{See the proposed rephrasing}


%%%%%%%%%%%%% fourth par %%%%%%%%%

To support the evaluation of PREGO, we review the procedural benchmarks of Assembly101~\cite{sener2022assembly101}  and Epic-tent~\cite{epicTent}, formalizing
%>> OLD:
%setting 
the novel task of online procedural mistake detection.
In the reviewed online
mistake detection
benchmarks, which we dub Assembly101-O and Epic-tent-O, the model is tasked with 
detecting when a procedural mistake is made, thus compromising the procedure.
%>>OLD:
%asserting when the procedure is compromised. 
This occurs when performing an action makes it impossible to complete the procedure without a correction procedure. 
% Note that multiple plausible ways may be available for procedures.\AL{questa frase sembra slegata dal contesto.}\AF{potremmo semplicemente rimuovere questa ultima frase}
The compromising mistake may be a wrong action or a relevant action performed in such an order that the action dependencies are not respected.

% \FG{Consider this version, which does not mention "first". I'd only mention "first" in Sec. 3. My suggested rewording: "In the reviewed online benchmarks, which we dub Assembly101-O and EpicTent-O, the model is tasked with asserting when the procedure is compromised, i.e.\ when performing an action makes it impossible to successfully complete the procedure (unless a correction procedure be adopted). Note that multiple plausible ways may be available for procedures. In fact, the compromising mistake may be a wrong action or a relevant action performed in such an order that the action dependencies be not respected."}
% In the reviewed online benchmarks, which we dub Assembly101-O and EpicTent-O, the model is tasked with asserting the occurrence of the procedural mistake as soon as it happens. While multiple procedures may be plausible, Assembly101-O and EpicTent-O mark as mistakes the first action, after which the procedure cannot be successful. 


% REMOVED text
% While original benchmarks contain mistake annotations, they have been designed for offline detection. 
% Therefore, they include multiple labeled mistakes beyond the first error. 
% To adapt these online detection benchmarks, we propose focusing exclusively on the first mistake in each procedural sequence. 
% This approach aligns with the real-world application of a mistake detector, which aims to detect and address errors as they occur rather than analyzing a complete sequence of multiple errors post-event.
% By concentrating on the first mistake, we can more accurately assess PREGO's efficacy and ability to prevent cascading errors in procedural tasks. 
% This modification also aligns the benchmarks with the practical needs of industries and domains where immediate error detection is crucial for maintaining process integrity and safety.
% This novel benchmark will serve as a more robust testing ground for PREGO and set a new standard for evaluating online procedural error detection models in future research.\FG{TO HERE.}


% Moreover, despite a challenging task, PREGO's results are particularly promising, underscoring its effectiveness and potential in advancing the field.
% \FG{I find these statements a bit tricky. Effectively the current datasets have corrective procedures, which we exclude. Saying that we exclude corrective procedures is not a bonus for us. I mean: we do it because it'd be difficult to also learn corrections, but it may be seen as our limitation, which should not have influenced our data preparation. My suggestion would be to stay away from statements on the detriments of multiple mistakes in a video. So take a positive writing perspective, proposing our review and motivating it.
% Effectively, our decision to consider the first mistake is a limitation, which we should acknowledge in a section for "limitations and future work", just before the conclusions.}
We summarize our contributions as follows:
\begin{itemize}
    \item We present PREGO, the first method designed for online and open-set detection of procedural errors in egocentric videos. PREGO's online feature ensures causal analysis by sequentially processing input videos up to a given frame, preventing future actions from influencing current step recognition.
    \item PREGO achieves open-setness by exclusively 
    relying on
    %OLD:
    %exposing it to 
    correct procedural sequences at training time, following the One-Class Classification (OCC) paradigm. This allows PREGO to identify a wide range of procedural mistakes, avoiding confinement to a predefined set of errors and avoiding the need for fine-grained mistake annotations.
    \item We propose using a pre-trained Large Language Model (LLM) for zero-shot symbolic reasoning through contextual analysis to predict the next action.
    \item To evaluate PREGO, we introduce the novel task of online procedural mistake detection and re-arrange existing dataset to provide two new
    %>>OLD:
    %in these 
    benchmarks, referred to as Assembly101-O and Epic-tent-O.
\end{itemize}


% \FG{Add a bulleted list of Contributions: "We summarize our contributions as follows:"..}




==> sec/Backup/2_rw_2023-11-05.tex <==
\section{Related Work}
\label{sec:relworks}



\AL{\begin{itemize}
    \item Procedural Learning
    \begin{itemize}
        \item trend topic
        \item some datasets are coming out with egocentric views and mistake annotations
        \item no one is handling the problem on both ego, OCC, and online
    \end{itemize}
    \item Egocentric Vision
    \begin{itemize}
        \item trend topics thanks to AR and VR systems.
        \item few works that works with egocentric videos aim to detect mistakes in procedural videos. No one is doing it in an OCC way.
    \end{itemize}
    \item OCC Video Anomaly Detection 
    \begin{itemize}
        \item Most recent Video anomaly detection methods work in an OCC scenario. They learn normality during train and detect anomalies during inference, assuming their unpredictability and open-setness. We differentiate from them since we're in a procedural setting, where the past context of actions counts to predict the actual anomaly. We're also ego, and no Video Anomaly detector is ego.
    \end{itemize}
\end{itemize}}

\ED{
\begin{itemize}
    \item Language Models
    \begin{itemize}
        \item Language Models (LMs) are statistical methods trained on large text corpora to learn the intricacies of human natural language.
        LMs predict the next words in a sentence, based on the context of the previous ones, and have shown abilities in various tasks.
        \item BERT (see below)
        % Pinpoint interesting advancements relevant to our model
        % \item GPT-based models % not sure if it is relevant.
        \item Due to the great importance of training data, in the last years models with billions of parameters have been trained on huge amounts of data, and the term Large LM (LLM) came of common use, even though it is inherently ambiguous and prone to change over time.
        These LLMs have great few-shot and zero-shot learning capabilities.
        \item Chat LMs (remove if we do not aim to report results on the anticipation with \textit{LM}-chat, also not sure if it is really needed).
    \end{itemize}
\end{itemize}
}
\LS{\begin{itemize}
    \item BERT
    \begin{itemize}
        \item BERT \cite{Devlin2019BERTPO}
        BERT, short for Bidirectional Encoder Representations from Transformers, is a Machine Learning (ML) model for natural language processing that was developed to assist computers in ‘understanding’ human language. BERT consists of two stages: pre-training and fine-tuning. Pre-training uses two self-supervised tasks: masked language modeling (MLM) and next sentence prediction (NSP). The NSP aspect of BERT teaches the model about sentence relationships by assessing whether a given sentence naturally succeeds the preceding one. Our research explicitly exploits this aspect of BERT.
        It is a prompt-based, few-shot learning approach that leverages an innovative pre-training task rooted in NSP. This task focuses on sentence-level pre-training for prompt understanding, accommodating variations in the length of label words. The effective utilization of NSP-BERT necessitates the creation of appropriate templates tailored to different tasks, thereby enhancing its zero-shot capabilities and facilitating more robust few-shot initialization.
    \end{itemize}
\end{itemize}}


\GD{\begin{itemize}
    \item Symbolic pattern Machines
    \begin{itemize}
        \item Large Language Models as General Pattern Machines \cite{generalpatternmachines2023}
        \item Plansformer: Generating Symbolic Plans using Transformers
        \item Recent work has explored the ability of LLMs such as GPT or Llama2 to operate as symbolic pattern machines. In this setting, LLMs can understand and solve problems when they are provided with a context within the same prompt that presents the problem in a zero-shot way without the need for further fine-tuning. We leverage this ability to make an LLM understand and continue sequences of symbolically represented steps in a procedure given examples of similar procedures. We differentiate from other works in two ways:
            \begin{enumerate}
                \item While \cite{generalpatternmachines2023} explores LLMs' ability to perform symbolic logic tasks, here we provide the model with sequences that do not follow a logic scheme but rather represent sequences of actions performed in a goal-oriented way, so that the model should be able to continue a sequence of symbols, given examples which make use of the same symbols, but that are not constrained in their ordering, nor there is a formula which can be found from the model to get the right answer.
                \item We adopt the LLM as a branch of the main model, coupling it with a second module that leverages the video source to predict the action played in the video. We then detect mistakes when the outputs of the two branches diverge. 
            \end{enumerate}
    \end{itemize}
\end{itemize}}

\LS{We could wrap BERT and Symbolic pattern machines under the LLM umbrella as a single section}
\ED{Agree on putting BERT and LLMs under the LM paragraph, but I'd leave symbolic reasoning as a stand-alone, to give it more relevance} \AL{we can put Procedural Learning and Egovision in the same section too}



==> sec/Backup/2_rw_2023-11-14.tex <==
\section{Related Work}
\label{sec:relworks}

% \FG{Attempt to define subsections based on all of your written notes. Feel free to modify titles and content. Bring material from the bullet into the subsections.}

\subsection{Procedural Datasets and Mistake Detection}
% \TODO{@Guido is iterating}\\
% \GD{\\Methods (eg Juan Carlos Niebles's work)\\
% Datasets\\
% How we relate (dataset): we modify two recent with mistakes to consider online and occ\\
% How we relate (dataset): we reason on procedural online, reasoning is symbolic, procedure graph is implicit}\\
Recent strides in procedural learning have spawned several datasets~\cite{ikea,epickitchens_Damen_2018,epicTent,salads,breakfasts,sener2022assembly101,coin,HoloAssist2023,IndustReal,proceL_2019,cross_task,howto100m_2019_miech}, 
% such as Meccano, EpicTent, Salads, 50Breakfasts, Assembly-101, COIN, HoloAssist, and Epic-Kitchen
 each giving unique insights into structured~\cite{sener2022assembly101,ikea,HoloAssist2023} and unstructured~\cite{epicTent,epickitchens_Damen_2018} task execution, from industrial assembly~\cite{Ragusa_meccano_2021,sener2022assembly101,IndustReal,ragusa2023enigma51} to daily cooking activities~\cite{epickitchens_Damen_2018,breakfasts,salads}. 
 Industrial-themed datasets typically provide egocentric views in controlled environments, while~\cite{coin,cross_task,howto100m_2019_miech} encompass a collection of publicly available instructional videos spanning several tasks. 
 Notably, \cite{sener2022assembly101,IndustReal,epicTent,HoloAssist2023} include error annotations crucial for mistake detection, where the primary challenge is identifying errors in a procedure's execution sequence.
 \FG{Separate two separate paragraphs on 1) datasets and 2) mistake detection. Name for 1: we relate to 1 as we resort to 2 datasets with mistake annotation, but we define the novel task of  online mistake detection. Name for 2: we're different from earlier because we're the first online and open-set} 
 However, the field lacks a unified approach to mistake detection, with fragmented literature and limited comprehensive evaluations. 
 \GD{here some comments on the baselines proposed by\cite{sener2022assembly101,IndustReal,epicTent,HoloAssist2023}} The notable exception is \cite{ding2023every}, which uses knowledge graphs for error identification. 
 It is worth noting that their method does not employ the video source, as it learns the procedures' steps directly from the transcripts of the procedures in~\cite{sener2022assembly101}. 
 Our work diverges as it leverages the video frames to detect the steps of the procedure and symbolic reasoning for an online assessment of the procedure's correctness.
\AL{we're not talking about egovision in the related works, which I think is one of the good points we have. We can incorporate this when talking about how we differentiate from the others.}


% \subsection{Egocentric action recognition and anticipation}
% \GD{Methods and datasets\\
% How we relate: use online SOTA OadTR, do not use anticipation (why?)\\
% }
% \AF{The sections on action recognition and anticipation of \href{https://openreview.net/forum?id=V3974SUk1w&noteId=BDo75NQgL0}{our survey} may be useful here}\GD{thanks for this very intriguing reference}

% Egocentric action recognition consists of identifying actions from the first-person perspective. It is functional in robotics and AR for context-aware assistance. Unlike exocentric (third-person) videos, egocentric videos present unique challenges due to the variable point of view and frequent occlusions where typically only the hands of the performer are visible. Early efforts in this domain leveraged Convolutional Neural Networks (CNNs)~\cite{synghetal_2016} and temporal sequence learning using Long Short-Term Memory networks (LSTMs), explored in~\cite{caoetal_2017}. \cite{kazakosetal_2019} introduced a fusion strategy integrating multiple modalities, such as audio and optical flow, to enhance network performance. \cite{plizzarietal_2022} leverage event camera data to overcome motion blur and improve temporal resolution. To benefit from the rich data available in third-person videos, \cite{Lietal_2021_EgoExo} proposed pretraining networks on these videos before applying them to egocentric action recognition tasks.
% Currently, \cite{Kazakosetal_2021} leads the state-of-the-art with an audio-visual transformer architecture incorporating a language model for improved action prediction. PREGO differs from these approaches as it employs a transformer Encoder to process the video stream, enhanced with an additional token that encodes previous actions to broaden the context window. 
% Action anticipation is a related task that aims at predicting the next action occurring after a certain frame in a video, given the context of previous frames. In the procedural setting, \cite{abufarha} proposed the long-term action anticipation task to forecast the next steps in a goal-driven procedure. Recently, \cite{epickitchens_Damen_2018, Furnari_2019} set the problem in the context of egocentric videos. PREGO encompasses an action anticipation branch, but it does not use any video clue. Instead, it leverages symbolic reasoning to interpret the output of the video recognition branch, and it anticipates the incoming actions provided with a context representing transcripts of correct procedures.
\subsection{Steps recognition and anticipation}

Step recognition is the task of identifying actions within a procedure. 
It is pivotal for understanding complex tasks such as autonomous robotics and educational technology. 
Recent contributions in this domain include \cite{Shah_2023_STEPs}, which uses a novel loss for self-supervised learning and a clustering algorithm to identify key steps in unlabeled procedural videos. 
\cite{POC_2022} introduces an action segmentation model using an attention-based structure with a Pairwise Ordering Consistency loss to learn the regular order of the steps in a procedure.
Notably, they devise a weakly supervised approach, using as labels only the set of actions occurring in the procedure, avoiding frame-level annotations. 
\cite{procedure_aware} approaches the task by leveraging online instructional videos to learn actions and sequences without manual annotations, blending step recognition with a deep probabilistic model to cater to the variability in step order and timing. 
PREGO differs from these approaches as it employs a transformer Encoder to process the video stream, enhanced with an additional token that encodes previous actions to broaden the context window.\FG{a bit surprising to read this, I assumed we used OadTR. So we would just state: we leverage the current SOTA, OadTR, for performing action recognition. One note: in this paragraph we should tell what we mean by "step", "action", "procedure". I assume the first two are synonyms, the third is a combination of the first two.}

On the other hand, step anticipation focuses on predicting forthcoming actions in a sequence crucial for real-time AI decision-making. 
\cite{Abdelsalam_2023_gepsan} addresses this by generating multiple potential natural language outcomes, pretraining on a text corpus to overcome the challenge of diverse future realizations. 
Additionally, \cite{self_regulated} framework proposes solutions to future activity anticipation in egocentric videos, using contrastive loss to highlight novel information and a dynamic reweighing mechanism to focus on informative past content, thereby enhancing video representation for accurate future activity prediction.
Unlike prior works, PREGO is the first model that anticipates actions via LLM symbolic reasoning in the label space.
% PREGO encompasses an action anticipation branch, but it does not use any video clue. Instead, it leverages symbolic reasoning to interpret the output of the video recognition branch, and it anticipates the incoming actions provided with a context representing transcripts of correct procedures.\FG{"PREGO differs from prior work as it's first to.." in this paragraph it's appropriate to make a clear statement, then may add "firs to anticipate next actions via LLM symbolic reasoning in the label space."}

% \subsection{Language modeling and next-token prediction}

% \FG{This subsection is out of scope. I'd remove it. Merge the statement on the extension of LMs to other tasks into the next subsection.}
% % LMs
% \AL{do we really need this section? I see some overlap with the In-context learning section. Maybe we can merge the two sections. If we keep this section alone, I'd emphasize more why we choose LLM for action anticipation and why we think it's the right way.}

% Language models (LMs) are statistical methods that aim to model the complexities of natural language by learning a distribution on large text corpora. 
% Given a sequence of past tokens, LMs are trained to predict the next one, which may be words or parts of words~\cite{radford2018improving, Devlin2019BERTPO}.
% Although this simple approach has shown great capabilities, this is mainly due to the size of the training data and the transformer architecture~\cite{vaswani2017attention}, which is specialized in learning complex relationships between features.

% LLMs
% In recent years, research in this area has scaled horizontally, moving towards data-based approaches in which transformer-based architectures with billions of parameters are fed huge quantities of data, resulting in further improvements~\cite{radford2019language, brown2020language}. 
% These LMs, which are sometimes referred to as large language models (LLMs), have shown even greater capabilities in modeling many natural language-related~\cite{touvron2023llama} and unrelated tasks~\cite{brooks2023instructpix2pix, Wei2022EmergentAO, gupta2023visual}.

% LLMs have recently been the center of attention, especially in their conversational variant~\cite{ouyang2022training, touvron2023llama}. 
% However, due to their possible misuse and computational limitations, whether they should be released to the public is currently under debate.

% We argue that there is a common ground between the next-token prediction mechanism of LMs and our action anticipation branch. 
% Therefore, we incorporate LMs into our pipeline by resorting to a state-of-the-art open-source model.

% \subsection{Symbolic reasoning}
\subsection{Large Language Models and In-context learning}
\TODO{@Edo iterating}

\FG{
% Call this section "Large Language Models and In-Context Learning". 
This subsection is all we need to say about LLMs. We just need to relate to techniques which take LLMs to other tasks and do so zero-shot'ly via in-context. One extra sentence which you may take from the previous subsection is one to witness of the growth of LLMs for other applications, beyond next word prediction.\\
EDIT: I notice we're missing a clear reference to symbolic reasoning, which we need to relate to. This may be added to the title eg "Large Language Modelling and Symbolic Reasoning". Then the content of this section can be (one paragraph per point): 1) widespread explotion of llm usage across a range of tasks, beyond next word prediction; 2) in-context learning, and few-/zero-shot learning; 3) symbolic reasoning.}

% As LLMs are trained on large training sets and employ a large number of parameters, new abilities emerged~\cite{Wei2022EmergentAO} i.e. compared to LMs, LLMs have shown new capabilities.
% Recent work has explored the ability of LLMs to operate as In-Context Learners (ICL), so as to be able to solve never-seen-before tasks. 
% In this setting, LLMs can understand and solve problems when they are provided with a context of input-output sequences 
% % within the same prompt \ED{I would omit it since we are not sure that it is common praxis to have the context in a single prompt, for sure we and LLMs as GPMs do}
% in a zero-shot manner without any need for further fine-tuning, to predict the output. 

% LLMs as ICL have been used for planning, programming, symbolic reasoning, or as general pattern machines.
% Some works have shown LLMs' ability to continue a semantically significant pattern; while others have explored LLMs in-context capabilities on semantically unrelated labels: in which there is no relation between a token and its meaning.

% We leverage ICL in our mistake detection pipeline, adopting the LLM in the action anticipation branch, continuing sequences of steps in a procedure, represented as symbols, given examples of similar procedures.
% Our LLM acts as a symbolic pattern machine, continuing the pattern of actions, given a context of sequences performed in a goal-oriented way, that do not follow a semantic scheme.
% Combining the challenges of predicting future actions and of having no semantics.
Large language models are trained on large datasets and have a large number of parameters. 
This gives them new capabilities compared to previous language models~\cite{Wei2022EmergentAO}.\\
LLMs have shown great capabilities in modeling many natural language-related~\cite{touvron2023llama} and unrelated tasks~\cite{brooks2023instructpix2pix, Wei2022EmergentAO, gupta2023visual}.
We argue that there is a common ground between their next-token prediction mechanism and our action anticipation branch.
Therefore, we incorporate LMs into our pipeline by resorting to a state-of-the-art model.

Recent research \AL{ref?} has explored LLMs' ability to operate as \textit{In-Context Learners} (ICLs), which means they can solve new tasks that they have never seen before. 
In this setting, LLMs can understand and solve problems when given a context of input-output sequences\GD{examples within the query prompt}, without any form of further fine-tuning.\\
LLMs as ICLs have been used for a variety of tasks, including planning~\cite{Pallagani2022PlansformerGS}, programming~\cite{gupta2023visual, Liang2022CodeAP}, and symbolic reasoning~\cite{generalpatternmachines2023}. 
Some work has shown that LLMs can continue semantically significant patterns~\cite{generalpatternmachines2023}, while other work has explored LLMs' in-context capabilities on semantically unrelated labels~\cite{Wei2023LargerLM}, where there is no relationship between a token and its meaning. 
Notably, recent research~\cite{Pallagani2022PlansformerGS,olmo2021gpt3} studied the opportunity to employ LLMs for devising plans to accomplish tasks. 
This is instrumental in robotics to enable automated entities to fulfill tasks.

In our mistake detection pipeline, we leverage ICL by using an LLM in the action anticipation branch. 
This LLM continues sequences of steps in a procedure, represented as symbols, given examples of similar procedures. 
Our LLM acts as a symbolic pattern machine, continuing the pattern of actions given a context of sequences performed in a goal-oriented way, even if the sequences do not follow a semantic scheme. 
This combines the challenges of predicting future actions and of having no semantics.

%Symbolic pattern machines\\
%How we relate: we argue this is the way, we propose their use for anticipation, for the first time
% \GD{\begin{itemize}
%     \item Symbolic pattern Machines
%     \begin{itemize}
%         \item Large Language Models as General Pattern Machines \cite{generalpatternmachines2023}
%         \item Plansformer: Generating Symbolic Plans using Transformers
%         \item Recent work has explored the ability of LLMs such as GPT or Llama2 to operate as symbolic pattern machines. In this setting, LLMs can understand and solve problems when they are provided with a context within the same prompt that presents the problem in a zero-shot way without the need for further fine-tuning. We leverage this ability to make an LLM understand and continue sequences of symbolically represented steps in a procedure given examples of similar procedures. We differentiate from other works in two ways:
%             \begin{enumerate}
%                 \item While \cite{generalpatternmachines2023} explores LLMs' ability to perform symbolic logic tasks, here we provide the model with sequences that do not follow a logic scheme but rather represent sequences of actions performed in a goal-oriented way, so that the model should be able to continue a sequence of symbols, given examples which make use of the same symbols, but that are not constrained in their ordering, nor there is a formula which can be found from the model to get the right answer.
%                 \item We adopt the LLM as a branch of the main model, coupling it with a second module that leverages the video source to predict the action played in the video. We then detect mistakes when the outputs of the two branches diverge. 
%             \end{enumerate}
%     \end{itemize}
% \end{itemize}}

% \AL{\begin{itemize}
%     \item Procedural Learning
%     \begin{itemize}
%         \item trend topic
%         \item some datasets are coming out with egocentric views and mistake annotations
%         \item no one is handling the problem on both ego, OCC, and online
%     \end{itemize}
%     \item Egocentric Vision
%     \begin{itemize}
%         \item trend topics thanks to AR and VR systems.
%         \item few works that works with egocentric videos aim to detect mistakes in procedural videos. No one is doing it in an OCC way.
%     \end{itemize}
%     \item OCC Video Anomaly Detection 
%     \begin{itemize}
%         \item Most recent Video anomaly detection methods work in an OCC scenario. They learn normality during train and detect anomalies during inference, assuming their unpredictability and open-setness. We differentiate from them since we're in a procedural setting, where the past context of actions counts to predict the actual anomaly. We're also ego, and no Video Anomaly detector is ego.
%     \end{itemize}
% \end{itemize}}

\subsection{Video anomaly detection}
\GD{Not sure if we need a section to compare our proposal with recent VAD literature. The relation would be in the OCC framework. On the other hand, we do not learn to classify correct steps, but we use only correct procedures as regular examples for in-context prediction. This relation would be stronger if we consider the action anticipation branch shaped as a video model, but we propose symbolic pattern machines which do not learn a normal class.}
\FG{Not sure how to anticipate reviewers here.. If I were a reviewer no.2, I'd say that errors are anomalies, open-set is a big thing in anomaly detection and several of those approaches are also online, so the novelty of this work is spoiled by that. I'd say: "Anomaly detection" is a better subsection title; the content below seems fine (I've edited the "how we relate"); make sure we answer the question: why are open-set online (video) anomaly detection techniques not applicable to solve error detection in procedures?}
\AF{Maybe - if we are not doing that already - we could put in the introduction a statement like ``... under these constraints, procedural mistakes can be seen as anomalies and online mistake detection can be framed as video anomaly detection. After all, PREGO is based on an anomaly detection assumption and if we clarify this, than considering state of the art methods for anomaly detection as baselines should be easy to understand.}
trend of open-set\\
embedding or reconstruction-based techniques\\
How we relate (maybe, TBD): AD and VAD do not scale to procedure-scales, we do so by LLMs (but watch out for techniques doing step anticipation at procedure scales, see if they relate to VAD)
%we extend a technique based on future prediction alignment (mocodad) to a heterogeneous dual stream model (video recog + symbolic reasoning)



==> sec/Backup/2_rw_2024-03-12.tex <==
\section{Related Work}
\label{sec:relworks}


\subsection{Procedural Datasets}

Recent progress in procedural learning has resulted in various datasets~\cite{ikea,epickitchens_Damen_2018,epicTent,salads,breakfasts,sener2022assembly101,coin,HoloAssist2023,IndustReal,proceL_2019,cross_task,howto100m_2019_miech,ragusa2023enigma51}, offering distinct insights into both structured~\cite{sener2022assembly101,ikea,HoloAssist2023} and unstructured~\cite{epicTent,epickitchens_Damen_2018} task execution. These datasets cover a range of activities, from industrial assembly~\cite{Ragusa_meccano_2021,sener2022assembly101,IndustReal,ragusa2023enigma51} to daily cooking~\cite{epickitchens_Damen_2018,breakfasts,salads}. Industrial datasets typically present egocentric views in controlled environments, while others~\cite{coin,cross_task,howto100m_2019_miech} comprise publicly available instructional videos across various tasks.
 
 Notably, \cite{sener2022assembly101,IndustReal,epicTent,HoloAssist2023} include error annotations crucial for mistake detection, where the primary challenge is identifying errors in a procedure's sequence. In this study, we use \cite{sener2022assembly101,epicTent} datasets since they give insights into errors happening during procedural in two different contexts, i.e., controlled industrial environments~\cite{sener2022assembly101} and open-air environments~\cite{epicTent}. In contrast to other benchmarks, we redefine procedural mistake detection as an open-set and online problem, aligning it more closely with real-world scenarios.
 \AL{we're introducing four references, but describing only \cite{sener2022assembly101}, why are we not using the others? I'd explain}
 % \FG{Separate two separate paragraphs on 1) datasets and 2) mistake detection. 
 % Name for 1: we relate to 1 as we resort to 2 datasets with mistake annotation, but we define the novel task of  online mistake detection. 
 % Name for 2: we're different from earlier because we're the first online and open-set} 
 \subsection{Procedural Mistake Detection}
 Despite the recent growing attention to procedural learning~\cite{sener2022assembly101,IndustReal,epicTent,HoloAssist2023} \AL{same references as the previous section but in this sentence we're talking about procedural learning.}, the field lacks a unified approach to mistake detection, with fragmented literature and limited 
 %>>OLD:
 %limited comprehensive 
 evaluations.   
 The notable exception is ~\cite{ding2023every}, which uses knowledge graphs for error identification. 
It is worth noting that~\cite{ding2023every} method does not employ the video source, as it learns the procedures' steps directly from the transcripts of the procedures in~\cite{sener2022assembly101}. 
Our work diverges \AF{from the aforementioned works} as it leverages the video frames to detect the steps of the procedure and symbolic reasoning for an online assessment of the correctness of the procedure. \AL{We're missing to describe Table 1 and how we differentiate from those methods.}
%>>OLD:
%process' correctness.



% \subsection{Egocentric action recognition and anticipation}
% \GD{Methods and datasets\\
% How we relate: use online SOTA OadTR, do not use anticipation (why?)\\
% }
% \AF{The sections on action recognition and anticipation of \href{https://openreview.net/forum?id=V3974SUk1w&noteId=BDo75NQgL0}{our survey} may be useful here}\GD{thanks for this very intriguing reference}

% Egocentric action recognition consists of identifying actions from the first-person perspective. It is functional in robotics and AR for context-aware assistance. Unlike exocentric (third-person) videos, egocentric videos present unique challenges due to the variable point of view and frequent occlusions where typically only the hands of the performer are visible. Early efforts in this domain leveraged Convolutional Neural Networks (CNNs)~\cite{synghetal_2016} and temporal sequence learning using Long Short-Term Memory networks (LSTMs), explored in~\cite{caoetal_2017}. \cite{kazakosetal_2019} introduced a fusion strategy integrating multiple modalities, such as audio and optical flow, to enhance network performance. \cite{plizzarietal_2022} leverage event camera data to overcome motion blur and improve temporal resolution. To benefit from the rich data available in third-person videos, \cite{Lietal_2021_EgoExo} proposed pretraining networks on these videos before applying them to egocentric action recognition tasks.
% Currently, \cite{Kazakosetal_2021} leads the state-of-the-art with an audio-visual transformer architecture incorporating a language model for improved action prediction. PREGO differs from these approaches as it employs a transformer Encoder to process the video stream, enhanced with an additional token that encodes previous actions to broaden the context window. 
% Action anticipation is a related task that aims at predicting the next action occurring after a certain frame in a video, given the context of previous frames. In the procedural setting, \cite{abufarha} proposed the long-term action anticipation task to forecast the next steps in a goal-driven procedure. Recently, \cite{epickitchens_Damen_2018, Furnari_2019} set the problem in the context of egocentric videos. PREGO encompasses an action anticipation branch, but it does not use any video clue. Instead, it leverages symbolic reasoning to interpret the output of the video recognition branch, and it anticipates the incoming actions provided with a context representing transcripts of correct procedures.
\subsection{Steps recognition and anticipation}

Step recognition is the task of identifying actions within a procedure. Indeed, a procedure is an ordered sequence of steps that bring to the completion of a task.
Step recognition is pivotal 
in areas
%>OLD:
%for understanding complex tasks 
such as autonomous robotics and educational technology. 
Recent contributions in this domain include \cite{Shah_2023_STEPs}, which uses a novel loss for self-supervised learning and a clustering algorithm to identify key steps in unlabeled procedural videos. 
\cite{POC_2022} introduces an action segmentation model using an attention-based structure with a Pairwise Ordering Consistency loss to learn the regular order of the steps in a procedure.
Notably, they devise a weakly supervised approach, using only the set of actions occurring in the procedure as labels, avoiding frame-level annotations. 
\cite{zhong_2023} approaches the task by leveraging online instructional videos to learn actions and sequences without manual annotations, blending step recognition with a deep probabilistic model to cater to the variability in step order and timing. 
% We leverage the current SOTA, OadTR, for performing action recognition. \AL{overclaim (?)}

On the other hand, step anticipation focuses on predicting forthcoming actions in a sequence crucial for real-time AI decision-making. 
\cite{Abdelsalam_2023_gepsan} addresses this by generating multiple potential natural language outcomes, pretraining on a text corpus to overcome the challenge of diverse future realizations. 
Additionally, the framework of~\cite{self_regulated}
%\cite{self_regulated} framework 
proposes solutions to future activity anticipation in egocentric videos, using contrastive loss to highlight novel information and a dynamic reweighing mechanism to focus on informative past content, thereby enhancing video representation for accurate future activity prediction.
Unlike prior works, PREGO is the first model that anticipates actions via LLM symbolic reasoning in the label space. \AL{maybe add more here?}
% PREGO encompasses an action anticipation branch, but it does not use any video clue. Instead, it leverages symbolic reasoning to interpret the output of the video recognition branch, and it anticipates the incoming actions provided with a context representing transcripts of correct procedures.\FG{"PREGO differs from prior work as it's first to.." in this paragraph it's appropriate to make a clear statement, then may add "firs to anticipate next actions via LLM symbolic reasoning in the label space."}

% \subsection{Language modeling and next-token prediction}

% \FG{This subsection is out of scope. I'd remove it. Merge the statement on the extension of LMs to other tasks into the next subsection.}
% % LMs
% \AL{do we really need this section? I see some overlap with the In-context learning section. Maybe we can merge the two sections. If we keep this section alone, I'd emphasize more why we choose LLM for action anticipation and why we think it's the right way.}

% Language models (LMs) are statistical methods that aim to model the complexities of natural language by learning a distribution on large text corpora. 
% Given a sequence of past tokens, LMs are trained to predict the next one, which may be words or parts of words~\cite{radford2018improving, Devlin2019BERTPO}.
% Although this simple approach has shown great capabilities, this is mainly due to the size of the training data and the transformer architecture~\cite{vaswani2017attention}, which is specialized in learning complex relationships between features.

% LLMs
% In recent years, research in this area has scaled horizontally, moving towards data-based approaches in which transformer-based architectures with billions of parameters are fed huge quantities of data, resulting in further improvements~\cite{radford2019language, brown2020language}. 
% These LMs, which are sometimes referred to as large language models (LLMs), have shown even greater capabilities in modeling many natural language-related~\cite{touvron2023llama} and unrelated tasks~\cite{brooks2023instructpix2pix, Wei2022EmergentAO, gupta2023visual}.

% LLMs have recently been the center of attention, especially in their conversational variant~\cite{ouyang2022training, touvron2023llama}. 
% However, due to their possible misuse and computational limitations, whether they should be released to the public is currently under debate.

% We argue that there is a common ground between the next-token prediction mechanism of LMs and our action anticipation branch. 
% Therefore, we incorporate LMs into our pipeline by resorting to a state-of-the-art open-source model.

% \subsection{Symbolic reasoning}
\subsection{Large Language Modelling and Symbolic Reasoning}
% \FG{
% Call this section "Large Language Models and In-Context Learning". 
% This subsection is all we need to say about LLMs. We just need to relate to techniques which take LLMs to other tasks and do so zero-shot'ly via in-context. One extra sentence which you may take from the previous subsection is one to witness of the growth of LLMs for other applications, beyond next word prediction.\\
% EDIT: I notice we're missing a clear reference to symbolic reasoning, which we need to relate to. This may be added to the title eg "Large Language Modelling and Symbolic Reasoning". Then the content of this section can be (one paragraph per point): 1) widespread explotion of llm usage across a range of tasks, beyond next word prediction; 2) in-context learning, and few-/zero-shot learning; 3) symbolic reasoning.}

Large language models are trained on large datasets and have many parameters. 
This gives them new capabilities compared to previous language models~\cite{Wei2022EmergentAO}.\\
LLMs have shown great capabilities in modeling many natural language-related~\cite{touvron2023llama} and unrelated tasks~\cite{brooks2023instructpix2pix, Wei2022EmergentAO, gupta2023visual}.
We argue that there is a common ground between their next-token prediction mechanism and our action anticipation branch.
Therefore, we incorporate LMs into our pipeline by resorting to a state-of-the-art model \AL{ref?}.

Recent research~\cite{Pallagani2022PlansformerGS, gupta2023visual, Liang2022CodeAP, Feng2023LanguageMC, generalpatternmachines2023} has explored LLMs' ability to operate as \textit{In-Context Learners} (ICLs), which means they can solve new tasks that they have never seen before. 
% LLMs can understand and solve problems in this setting when given a context of input-output sequences\GD{examples within the query prompt}, without further fine-tuning.
Given a query prompt with a context of input-output examples, LLMs can comprehend and address the problems in this setting without further fine-tuning.




LLMs as ICLs have been used for a variety of tasks, including planning~\cite{Pallagani2022PlansformerGS}, programming~\cite{gupta2023visual, Liang2022CodeAP}, logical solvers~\cite{Feng2023LanguageMC}, and symbolic reasoning~\cite{generalpatternmachines2023}. 

Some work has shown that LLMs can continue semantically significant patterns~\cite{generalpatternmachines2023}, while other work has explored LLMs' in-context capabilities on semantically unrelated labels~\cite{Wei2023LargerLM}, where there is no relationship between a token and its meaning. 
Notably, recent research~\cite{Pallagani2022PlansformerGS,olmo2021gpt3} studied the opportunity to employ LLMs for devising plans to accomplish tasks. 
This is instrumental in robotics to enable automated entities to fulfill tasks.
In our mistake detection pipeline, we leverage ICL using an LLM in the action anticipation branch. 
This LLM continues sequences of steps in a procedure, represented as symbols, given examples of similar procedures. 
Our LLM acts as a symbolic pattern machine, continuing the pattern of actions given a context of sequences performed in a goal-oriented way, even if the sequences do not follow a semantic scheme. 
This combines the challenges of predicting future actions and of having no semantics.

%Symbolic pattern machines\\
%How we relate: we argue this is the way, we propose their use for anticipation, for the first time
% \GD{\begin{itemize}
%     \item Symbolic pattern Machines
%     \begin{itemize}
%         \item Large Language Models as General Pattern Machines \cite{generalpatternmachines2023}
%         \item Plansformer: Generating Symbolic Plans using Transformers
%         \item Recent work has explored the ability of LLMs such as GPT or Llama2 to operate as symbolic pattern machines. In this setting, LLMs can understand and solve problems when they are provided with a context within the same prompt that presents the problem in a zero-shot way without the need for further fine-tuning. We leverage this ability to make an LLM understand and continue sequences of symbolically represented steps in a procedure given examples of similar procedures. We differentiate from other works in two ways:
%             \begin{enumerate}
%                 \item While \cite{generalpatternmachines2023} explores LLMs' ability to perform symbolic logic tasks, here we provide the model with sequences that do not follow a logic scheme but rather represent sequences of actions performed in a goal-oriented way, so that the model should be able to continue a sequence of symbols, given examples which make use of the same symbols, but that are not constrained in their ordering, nor there is a formula which can be found from the model to get the right answer.
%                 \item We adopt the LLM as a branch of the main model, coupling it with a second module that leverages the video source to predict the action played in the video. We then detect mistakes when the outputs of the two branches diverge. 
%             \end{enumerate}
%     \end{itemize}
% \end{itemize}}

% \AL{\begin{itemize}
%     \item Procedural Learning
%     \begin{itemize}
%         \item trend topic
%         \item some datasets are coming out with egocentric views and mistake annotations
%         \item no one is handling the problem on both ego, OCC, and online
%     \end{itemize}
%     \item Egocentric Vision
%     \begin{itemize}
%         \item trend topics thanks to AR and VR systems.
%         \item few works that works with egocentric videos aim to detect mistakes in procedural videos. No one is doing it in an OCC way.
%     \end{itemize}
%     \item OCC Video Anomaly Detection 
%     \begin{itemize}
%         \item Most recent Video anomaly detection methods work in an OCC scenario. They learn normality during train and detect anomalies during inference, assuming their unpredictability and open-setness. We differentiate from them since we're in a procedural setting, where the past context of actions counts to predict the actual anomaly. We're also ego, and no Video Anomaly detector is ego.
%     \end{itemize}
% \end{itemize}}



% \subsection{Video anomaly detection}
% \GD{Not sure if we need a section to compare our proposal with recent VAD literature. The relation would be in the OCC framework. On the other hand, we do not learn to classify correct steps, but we use only correct procedures as regular examples for in-context prediction. This relation would be stronger if we consider the action anticipation branch shaped as a video model, but we propose symbolic pattern machines which do not learn a normal class.}
% \FG{Not sure how to anticipate reviewers here.. If I were a reviewer no.2, I'd say that errors are anomalies, open-set is a big thing in anomaly detection and several of those approaches are also online, so the novelty of this work is spoiled by that. I'd say: "Anomaly detection" is a better subsection title; the content below seems fine (I've edited the "how we relate"); make sure we answer the question: why are open-set online (video) anomaly detection techniques not applicable to solve error detection in procedures?}
% \AF{Maybe - if we are not doing that already - we could put in the introduction a statement like ``... under these constraints, procedural mistakes can be seen as anomalies and online mistake detection can be framed as video anomaly detection. After all, PREGO is based on an anomaly detection assumption and if we clarify this, than considering state of the art methods for anomaly detection as baselines should be easy to understand.}
% \FG{If we have a comparison with SOTA VAD or AD techniques in our tables, then it's all fine. If we don't have the direct comparison, but if there are techniques which are online and open-set, then we might be in trouble. They may say we should have reviewed and compared to that literature, too. If we don't have those techniques in our tables, and if it's late to arrange for it, then the comment below on the procedural challenge of large-scale / long-term reasoning / currently not viable training on this frame length might be a way to avoid this issue.}\\
% trend of open-set\\
% embedding or reconstruction-based techniques\\
% How we relate (maybe, TBD): AD and VAD do not scale to procedure-scales, we do so by LLMs (but watch out for techniques doing step anticipation at procedure scales, see if they relate to VAD)
%we extend a technique based on future prediction alignment (mocodad) to a heterogeneous dual stream model (video recog + symbolic reasoning)



==> sec/Backup/3_meth-2024-03-12.tex <==
\section{The PREGO Model}
\label{sec:methodology} 


% \FG{+1}


Our framework for online mistake detection exploits a dual-branch architecture that integrates procedural step recognition with anticipation modeling, as depicted in Fig.~\ref{fig:conceptual}
% \FG{this should now refer to the teaser, I imagine. Here we name the framework}. 
% The primary branch focuses on online step recognition within ongoing tasks, employing egocentric video data to monitor workers' actions. This branch processes each frame sequentially, assigning a classification to individual frames. This classification is inherently online, relying solely on historical frame data to determine the present step, thus avoiding any reliance on future frame information. The output of this process is a temporally bound sequence of steps, representing the actions in the procedure up to a specific time point \(t_0\).
% The secondary branch of our architecture employs an LLM, Llama2, for anticipating the next steps via symbolic reasoning. This branch is responsible for processing the sequence of steps encoded symbolically (with textual step descriptors transposed into numerical identifiers) to forecast the ensuing procedural step. This predictive function is executed by inputting the step sequence derived from the first branch into Llama2\cite{touvron2023llama}, complemented by a context of correctly executed procedural sequences for the same task encoded symbolically within the same prompt. Notably, this process leverages the zero-shot learning capabilities of Llama2\cite{touvron2023llama}, obviating the need for explicit fine-tuning of the model. This approach underscores the scalability and adaptability of our system to a diverse array of procedural contexts. Finally, we can detect mistakes by comparing the output of the two branches on the same frame, deeming the mismatches as mistakes. 
In the following sections, we elaborate on the problem formalization (Sec. \ref{sec3:prego}), present the branches for step-recognition (Sec. \ref{sec3:oadtr}) and step-anticipation (Sec. \ref{sec3:symb}), and finally we illustrate the mistake detection procedure (Sec. \ref{sec3:mistake}).
% In this section, we start by defining the problem, followed by a comprehensive explanation of PREGO (Sec. \ref{sec3:prego}). We will initially focus on its video component for step classification (Sec. \ref{sec3:oadtr}) and subsequently explore its application in symbolic language modeling (Sec. \ref{sec3:symb}) for step anticipation. Lastly, we use both for mistake detection (Sec. \ref{sec3:mistake}).
% \AF{Maybe it could be useful to reference a figure when we mention the ``dual-branch'' architecture.}


\subsection{Problem Formalization}
\label{sec3:prego}
We consider a finite set of $N$ procedures %$\mathcal{P}=$
$\{p_i\}_{i=1}^N$ 
% which come with a transcript $\mathcal{G}=\{g_i\}_{i=1}^N$ 
% \GF{we use T as subscript of frames later. Can be useful to change the name of this set to avoid confusion} 
that encodes the sequence of actions as $p_i = \{ a_k\}_{k=1}^K $ where $K$ varies depending on the specific procedure and $a_k \in \mathcal{A}= \{a | a \text{ is a possible action }\}$.
%by means of the , given a set of possible action steps $\mathcal{A}=\{a_1,a_2,\dots, a_K\}$, encode the sequence of actions encompassed by the procedure.
Each procedure is also represented by a set of videos 
%video %${v_{p_i}\}_{i=1}^N=
$\{v_i\}_{i=1}^N$
% \\ (\AF{is it a single video per procedure or a set of videos? - shall we use the $j$ subscript here to avoid confusion with the $p_i$?}\GD{Actually I wanted to stress it since the video, the procedure, and the transcript are associated, as they describe the same ``concept"})\\
that, in turn, 
are
%is 
composed of frames $v_i=\{f_\tau\}_{\tau=1}^{M_i}$ where $M_i$ is the total number of frames in the video $i$.
\\Fixed a frame $f_{\bar{\tau}}$ from a given video $v_{\bar{i}}$, PREGO's task is double-folded: it has to (1) recognize the action $a_{\bar{\tau}}$ corresponding to the frame $f_{\bar{\tau}}$ in the video and (2) predict
% anticipate \GF{probably it is better if we refer this as prediction and not anticipation...since the action is happening during this prediction} 
the action $a_{\bar{\tau}}$ that will take place 
% shortly \GF{will take place at time $\bar{\tau}$  considering past observation until time $\bar{\tau}-1$ }
at time $\bar{\tau}$ considering only past observations until time $\bar{\tau}-1$.
% past observations until time $\bar{\tau}-1$.
\\The step recognition task is performed by a module $\rho$ that takes as input the encoded frames of $v_{\bar{i}}$ up to $\bar{\tau}$ and returns an action $a^{\rho}_{\bar{\tau}}$. 
%We then collect all the $\rho$ predictions for $v_{\bar{i}}$ and represent them as a transcript $\hat{g}_{\bar{i},\bar{\tau}-1}$ up to time $\bar{\tau}-1$.
We then feed the module $\xi$, responsible for the anticipation task, with all the $a^{\rho}_1, ...,a^{\rho}_{\bar{\tau}-1} $ actions to have a prediction $a^{\xi}_{\bar{\tau}}$ for the next action in the obtained sequence.
\\Finally, we compare $a^{\rho}_{\bar{\tau}}$ with $a^{\xi}_{\bar{\tau}}$
and we deem as mistaken the actions 
where a misalignment between the outputs of the two branches occurs. For the sake of clarity, in the remainder of this section, we consider a single procedure \(p\) associated with a video \(v\) . %and a transcript \(g\). 
 %\\ (\AF{Shall we say ``we deem as mistaken ... if?'' - Do we generate a ``mistake'' score or are we just predicting mistakes in a binary fashion?}\GD{binary fashion (mistake detected after mismatch)}).
% In our online setup, we causally analyze the video, predicting procedural mistakes for each frame based on information from previous frames (see Fig.~\ref{fig:frame_pic}). 
% The problem is also defined as open-set, where mistakes observed during testing have not been seen during training.
% We begin with a video input represented as $V = {\{f_t\}}_{t=0}^{T}$, where $f_t$ is the $t^{th}$ frame of the video. Our initial step involves classifying the steps of the procedures $p_{V,t}$ for each frame $f_t$. We then employ symbolic pattern machines to detect errors.
% %, represented as $m$. 

% We extract a chunk $c$ of frames $f_C$, where $C = \{t, \ldots, c\}$ to perform the classification task. 
% We then classify $f_C$ and obtain a predicted step of a procedure $\hat{p}_c$ for the last frame considering $f_c$. The predicted procedure, $\hat{p}_c$, takes values from the set $P = \{0, \ldots, N\}$, where $N$ is the total number of action categories (detailed in Sec. \ref{sec3:oadtr}).

% Next, we proceed with the error detection process, employing symbolic pattern machines as detailed in \cite{generalpatternmachines2023}. We take the predicted classes, denoted as $\hat{p} = \{\hat{p}_0, \ldots, \hat{p}_{c-1}\}$, and execute sequence completion to generate $\tilde{p}_c$ (detailed in Sec. \ref{sec3:symb}).

% Once we have both the predicted class $\hat{p}_c$ and the completed sequence $\tilde{p}_c$, we compare the two. If they match, we deem the procedure correct; otherwise, it is incorrect.

% \LS{I Wrote the symbolic part as intra-step predictor. Should I re-write it as a last-step predictor?}

\subsection{Step Recognition}
\label{sec3:oadtr}
\AL{I find this section extremely confused. We need to introduce the method and the losses used for the step recognition part.}
% \AL{in the intro we're using the terms "Action Anticipation" and "Action Recognition" to define the two branches. I'd rename sec 3.2 and 3.3 following that naming. I think it's easier for the reviewer to follow our narration.}
% \LS{I renamed the subsections to step recognition and anticipation following the related work. I agree with you Ale, we should be consistent throughout.}
% As in \cite{OadTR}, we adopt the feature extraction procedure of \cite{TSN}, which transforms a chunk composed of \(W\) consecutive frames $ \{f_w\}_{w=1}^W$into a $1$D feature sequence by representing frames with Convolutional Nerual Networks and collapsing the spatial dimensions. Subsequently, a linear projection layer projects each frame chunk into a $D$-dimensional feature space resulting in the token sequence  $F = \{token_i\}_{i=t}^{W} \in \mathbb{R}^{W \times D}$. We then utilize the encoder introduced in \cite{OadTR}, where Multi-head self-attention is the key component of the Transformer. At its core, self-attention revolves around the concept that individual tokens have the ability to engage with and acquire valuable semantic information from other tokens, enhancing their ability
% %capacity 
% to capture extensive relationships. This quality makes it highly adept at capturing long-distance dependencies. Finally the output representation of the encoder corresponding to the predicted procedure $\hat{p}_c$ (as in the upper part of Fig. \ref{fig:frame_pic}) (\AF{``Finally the out representation of the encoder corresponing to ...'' This sentence seems to be incomplete'')}. 

% \LP{NEW VERSION}
We capitalize on the established OadTR \cite{OadTR} encoder  that leverages the Transformers capabilities for online action detection to build our recognition branch. If fact, even if it is possible to make recognition using the encoder-decoder architecture, 
%\GD{Introduce the edits on the original~\cite{OadTR}} 
we show in Fig.~\ref{fig: mAP Encoder vs Encoder-Decoder} that the model benefits from having only the encoder module when coupled with a larger window W that includes more frames to produce its prediction. This choice leads to a better mAP considering different values for the window length and a drastic reduction of the parameters (\(\sim 1/3\)) compared to the original model.

In this setup, defining $w$ as the size of the window W, the model predicts the action $a_{\tau}$ considering the frames $\{f_{{\tau}-w},..,f_{\tau}\}$. This mechanism produces redundant results since the model eventually predicts the same action for consecutive frames. In order to obtain a consistent procedure, we simply consider unique actions every time the prediction for consecutive frames is the same.



\subsection{Step Anticipation}
\label{sec3:symb}
We introduce a novel approach for step forecasting in procedural learning by harnessing the power of symbolic reasoning~\cite{generalpatternmachines2023} through a Language Model (LM). Specifically, we employ a Large Language Model (LLM) for next-step prediction, feeding it with prompts constructed from procedural video transcripts. These prompts are structured in two parts: the first part comprises contextual transcripts \(CT\) \AL{why CT? is it C instead?}
extracted from similar procedures to inform the LLM about typical step sequences and order. 
% We extract CT from the correct procedures split, 
The second part includes the current sequence of actions up to a specific frame, \(f_{\bar{\tau}}\), detected by our module $\rho$, i.e., 
\begin{equation}
%\rho(v|_{\bar{\tau}})= \hat{g}=[\hat{a}^{\rho}_{1}, \hat{a}^{\rho}_{2},...\hat{a}^{\rho}_{T-1}].  
g_{\bar{\tau}} = [a^{\rho}_{1},...,a^{\rho}_{\bar{\tau}-1}] 
\end{equation}
This approach enables the LLM to utilize in-context learning, eliciting its ability to anticipate subsequent actions. Our framework operates in a zero-shot fashion, relying on the LLM's ability to retrieve the correct sequence continuation without specific training or fine-tuning but only leveraging the positive examples within the input prompts. Additionally, our method employs symbolic representations of the steps, converting the set of actions $\mathcal{A}$ into a symbolic alphabet $\Omega$ through an invertible mapping $\gamma$. Therefore, we can express the symbolic predicted sequence as:
\begin{equation}
%\gamma(\hat{g})=[\gamma(\hat{a}^{\rho}_{1}), \gamma(\hat{a}^{\rho}_{2}), ..., \gamma(\hat{a}^{\rho}_{T-1})].
\gamma(g_{\bar{\tau}})=[\gamma(a^{\rho}_{1}), ..., \gamma(a^{\rho}_{\bar{\tau}-1})]=[\omega_1, ..., \omega_{\bar{\tau}-1}]
\end{equation}
This conversion abstracts the actions from their semantic content, allowing the LLM to focus on pure symbols and sequences, thus simplifying the complexity of predicting the following action. \\ 
Finally, the \(\xi\) module, given the examples \(C\) \AL{is this C referred to the CT introduced above?} and the current symbolic transcript \(\gamma(g_{\bar{\tau}})\) described in its prompt, is required to output the most probable symbol $\omega_{\bar{\tau}}$ to continue the sequence.
%\begin{equation}
%    \xi(CT,\gamma(g_{\bar{\tau}}) )= a^{\xi}_{ \bar{\tau}} \gamma(a^{\xi}_{i, T})
%\end{equation}
At this point, we apply the inverse function of $\gamma$ to retrieve the underlying step label, i.e.,  \(a^{\xi}_{\bar{\tau}} = \gamma^{-1}( \omega_{\bar{\tau}})\). \AL{I'd point to figure 2 in the text. The figure needs to have the same nomenclature defined here.}
%\AF{In che senso è invertita? $^{-1}$ fa pensare a un reciproco $1/x$, ma immagino che non sia questa l'operazione alla quale ci riferiamo.}
% \GD{introduce $\xi(C,\gamma(\hat{g_i}))=\hat{a}^{\xi}_{i, T}$}

% Following \cite{generalpatternmachines2023}, we employ symbolic reasoning of LLMs for sequence transformation and customize it to suit our specific scenario.
% We exploit the ability of LLMs to acquire an understanding of the distribution of functions that depict sequence transformations in context.
% \AF{The last sentence is redundant with the previous one.} This is achieved by identifying and extrapolating abstract patterns present within instances of input-output sequences, where each element is selected from a diverse set of tokens originating from a predetermined alphabet $\mathcal{A}$, where in our case are a subset of possible procedures $P$ (\AF{This last part is a bit confusing (from the second ``where''. Does it mean that A is a subset of procedure? Or the input-output sequences are a subset of procedures? Should it be a subset of videos?}).
% Our prompt is a collection of input-output sequences of correct procedures $p=(p_{(0:c-1)}^{in}, p_{c}^{out})$ (\AF{In the problem formalization we distinguish between procedures and videos. In my understanding a procedure is a description of how the task should be carried out - hence a ``transcript'' - i.e., list of steps without temporal grounding - is associated. The videos instead are realizations of the procedures. Is my understanding correct? If so, then, in this case, are we passing procedures or video labeles as examples?}) as context for the LLM to understand. Then we conclude the prompt with $\hat{p}$ expecting $\tilde{p}_c$. \AF{what we mean by ``we conclude the prompt''?}


\subsection{Mistake Detection}\label{sec4:PMD_formal}
We finally compare the outputs of the two modules to detect procedural mistakes. Precisely, we consider as correct all the steps where the outputs of the two modules align with each other, while we deem as an error the cases for which the two outputs diverge. That is:
\begin{equation}
\begin{cases}
    a^{\rho}_{\bar{\tau}} \neq a^{\xi}_{\bar{\tau}} & \text{MISTAKE} \\
    a^{\rho}_{\bar{\tau}} = a^{\xi}_{\bar{\tau}} & \text{CORRECT} \\
\end{cases}
\end{equation}
\label{sec3:mistake}



% \subsection{Implementation}
% Describe what is trained, what is zero-shot etc






==> sec/Backup/3_meth_2023-11-05.tex <==
\section{Methodology}
\TD{Brief outline of approach
\begin{itemize}
    \item using bullets
    \item A brief outline of the approach we follow or propose
\end{itemize}}


==> sec/Backup/3_meth_2023-11-07.tex <==
\section{PREGO}
\TODO{@Luca is iterating}

% \FG{Attend to define subsections. My idea: since we assemble two big pieces that were never together (video recog and symbolic reasoning), we start from our proposal of framework.}
In this section, we will start by defining the problem, followed by a comprehensive explanation of PREGO (Sec. \ref{sec3:prego}). We will initially focus on its video component for frame classification (Sec. \ref{sec3:oadtr}) and subsequently explore its application in symbolic language modeling (Sec. \ref{sec3:symb}) for mistake detection.

\paragraph{Problem definition}
In our online setup, we causally analyze the video, predicting mistakes for each frame based on information from previous frames. The problem is also defined as open-set, where mistakes observed during testing may not have been seen during training.
Our primary objective is to detect procedural errors denoted as $m$ in procedural videos represented as $V$. \AF{This is the only notation appearing in this paragraph. It could be worth to extend it a bit or remove it completely, if we think it is clear enough without notation.}
\LS{need to incorporate OCC}. \AF{Since we're going to have a section on the benchmark, would it make sense to have this problem definition there? Maybe not, if the benchmark section will come after the current one.}

\AF{One alternative approach for this section could be: let's bring all possible notation here, then we refer to the same notation in the next sections. For instance, ``Given a video $V=\{f_t\}_{t=0}^T$, where $f_t$ is the $t^{th}$ frame and the video has $T$ frames in total, we define online procedural mistake detection as the task of ...''. We then do not need to repeat the $f_t$ notation where needed.}

\subsection{Online procedural mistake detection}
\label{sec3:prego}
We begin with a video input represented as $V = {\{f_t\}}_{t=0}^{T}$, where each $f$ corresponds to an individual frame (\AF{where $f_t$ is the $t^{th}$ frame of the video)}. Our initial step involves classifying procedures as $p$ at the frame level $f$ (\AF{making predictions $p_t$ for each frame $f_t$? - what kind of predictions are these? mistakes? or maybe actions?}). We then employ symbolic pattern machines to detect errors, represented as $m$. 

To perform the classification task, we extract a chunk of frames $f_C$, where $C = \{t, \ldots, c\}$ and $c$ are determined by adding the window size to the current $t$ frame \AF{what do we mean by ''adding the window size''?}. We then classify this chunk of frames (\AF{each chuck $F_C$?}) and derive a predicted procedure $\hat{p}_c$ (\AF{what do we mean by ``derive a predicted procedure''}) for the last frame considering $f_c$. The predicted procedure, $\hat{p}_c$, takes values from the set $p = \{0, \ldots, N\}$, where $N$ signifies (\AF{is}) the total number of action categories.

Next, we proceed with the error detection process, employing symbolic pattern machines as detailed in [cite]. We take the predicted classes, denoted as $\hat{p} = \{\hat{p}_0, \ldots, \hat{p}_{c-1}\}$, and execute sequence completion to generate $\tilde{p}_c$.

Once we have both the predicted class $\hat{p}_c$ and the completed sequence $\tilde{p}_c$, we compare the two. If they match, we deem the procedure correct; otherwise, it is incorrect.

\LS{Wrote the symbolic part as intra-step predictor. Should I re-write it as a last-step predictor?}

\subsection{Frame Classisfication}
\label{sec3:oadtr}
\AF{I found this section and the previous one (Online procedural mistake detection) a bit overlapped. Would it make sense to merge them? Also, an initial reference to a figure will help a lot. We can then shape subsections depending on the modules appearing in the figure.}
We initiate our process with a streaming video denoted as $V = \{f_t\}_{t=0}^{T}$. The feature extraction, as described in \LS{Cite}, (\AF{we adopt the feature extraction procedure of [], which}) transforms this video into a 1D feature sequence by collapsing the spatial dimensions. Subsequently, a linear projection layer further maps each vectorized frame chunk feature into a $D$-dimensional feature space. The resulting token sequence is represented as $F = \{ \text{token}_t \}_{t=0}^{T} \in \mathbb{R}^{(T + 1) \times D}$.

Within the encoder, we extend a trainable token class, $\text{token}_\text{class} \in \mathbb{R}^D$, to incorporate it into the embedded feature sequence $F$, resulting in the combined token feature sequence $\tilde{F} = \text{Stack}(\{ \text{token}_t \}_{t=0}^{T}, \text{token}_\text{class}) \in \mathbb{R}^{(T + 2) \times D}$. It's essential to note that $\text{token}_\text{class}$ serves the purpose of learning global discriminative features relevant to the online action detection task.
\LS{Add citation OadTR and TSN. Say how we differentiate from OadTR and add novelty part of text token which focuses on context}


\subsection{Mistake Detection - Symbolic Pattern Machines}
\label{sec3:symb}
Describe the technique of [x]. Referring to it once is fine. We describe the important high level details

\subsection{Implementation}
Describe what is trained, what is zero-shot etc






==> sec/Backup/4_exp-2024-03-12.tex <==
\section{Experiments}
\label{sec:experiments}

% \input{Tables/assembly_PREGO}
% \input{Tables/epicTents_PREGO}
\input{Tables/assembly_epic_together}
In this section, we present the results of our experiments on online and open-set mistake detection in procedural videos. We contrast PREGO with several baselines that employ different mistake detector techniques or use part of the ground truth as an oracle. 
% \LP{I would not mention the oracle in this section and in table 2, but i would leave it for a specific section in 6 Ablation studies. In this way all the results in table 2 are comparable and make sense }. 
All the baselines are assessed on the Assembly101-O and Epic-tent-O datasets, detailed in section \ref{sec4:datasets}. The metrics used are F1 score, precision and recall, explained in \ref{sec4:metrics}. We first describe the baselines in section \ref{sec:baselines}, and then analyze the results in \ref{sec:results}, \AL{I'd remove: shown in Table \ref{tab:together}}.


\subsection{Baselines}
\label{sec:baselines}

% \FG{Add an intro: "We compare PREGO against the following baselines:}

\noindent To estimate the effectiveness of PREGO, we evaluate its performance  by comparing it against the following baseline models based on the metrics presented in Sec.~\ref{sec4:metrics}:

\myparagraph{One-step memory} We define a {\it transition matrix} considering only the correct procedures. Specifically, given the set of the actions  $\mathcal{A}$ in the training set with $|\mathcal{A}|=C$, we define a transition matrix $M\in\mathbb{R}^{C\times C}$ 
% where  we annotate the occurrences of the bi-grams of actions in the corrected split of procedures \LP{possible rephrasing: we define a transition matrix $M\in\mathbb{R}^{C\times C}$ 
which stores in position $(l,m)$ the occurences that action $m$ follows action $l$. 
% }. 
We then label as {\it mistake} the actions occurring in the test split that do not correspond to transitions recorded in the training set.
% not admitted by the matrix $M$. \todo{In che senso ``not admitted''? È una baseline absata su GT?}

% \myparagraph{Bayesian Personalized Ranking (BPR)} 
% % \AL{@Guido check this again. If good remove this comment.} 
% In addressing the inherent sparsity of the matrix $M$, we draw inspiration from collaborative filtering methods commonly employed in approximating User-Item matrices in the domain of recommendation systems. Precisely, we adopt the Bayesian Personalized Ranking (BPR)\cite{BPR} as a matrix factorization technique. By considering bi-grams of actions, we fit a BPR model to the transition matrix $M$, interpreting actions as users and items. Given an initial action, the model recommends a top-\(k\) list of subsequent actions. An action is deemed \textit{correct} if it naturally follows the initial action and appears in the BPR-recommended list; otherwise, it is marked as a \textit{mistake}. 
% \AF{Here we could mention that we consider this as a more sophisicated version of the frequentist baseline.}


\myparagraph{OadTR for mistake detection}
%\FG{it might be better to rename the anticipating OadTR as OadTR-A, or any other. The point is that OadTR is used earlier and later for recognition. In any case shifting labels defines a new method, it might be clearer} 
\cite{OadTR} proposes a framework for online action detection called
% , which is the task of recognizing actions in videos as they occur. 
 % The framework, named 
OadTR that
% , 
employs Transformers to capture the temporal structure and context of the video clips. The framework consists of an encoder-decoder architecture. The encoder takes the historical observations as input and outputs a task token representing the current action. The decoder takes the encoder output and the anticipated future clips as input and outputs a refined task token incorporating the future context.
%\AF{La descrizione generale di OadTR credo che possa essere evitata per risparmiare spazio} We modify OadTR to detect procedural mistakes in the online open-set Procedural Mistake Detection setting by examining the difference between the step recognition (encoder) and step anticipation (decoder) branches. 
% \LP{ possible rephrasing: In this setting, a misalignment between the actions predicted by the encoder and by the decoder branches respectively produces a mistake.} 
%A discrepancy signifies that either one or both branches have made an erroneous prediction of the action class, which implies an input context that diverges from the normal procedures that were learned during the training phase.
% \LP{NEW VERSION:}
% \cite{OadTR} proposes OadTR, a framework for online action detection that employs Transformers to capture the temporal structure and context of the video clips. The framework consists of an encoder-decoder architecture. Drawing inspiration from OadTR, we create a Double-Encoder OadTR that is thought for mistake detection task that is a totally video-based counterpart of PREGO. It employs a dual encoder architecture that performs action recognition in one branch and action prediction in the other. To find if a mistakes is present at time $\bar{\tau}$, the model considers as input the window including the frame to be recognized $f_{\bar{\tau}-w},...,f_{\bar{\tau}}$ in the recognition branch and the same window masked to exclude the current frame $f_{\bar{\tau}-w},...,f_{\bar{\tau}-1}$ in the prediction branch. 
A discrepancy between the outputs of the encoder and the decoder produces a mistake




\myparagraph{BERT~\cite{Devlin2019BERTPO}}
%\FG{maybe start with "We leverage the capability of BERT and its specific [CLS] token for predicting the correct or mistaken sequence of actions. In more details.." please check this wording}
We leverage the capability of BERT utilizing its specific [CLS] token to predict the correct or erroneous sequence of action. More specifically, we fine-tune BERT using the next-sentence-prediction task, where the model is trained to predict whether one sentence logically follows another within a given text. In our context, we apply this to determine whether step B can follow another step A within a procedure. Here, steps are defined as sets of two words, such as \textit{attach wheel}, representing coarse actions. To execute this, BERT is presented with pairs of sentences corresponding to procedures A and B, tasking it with predicting the sequential relationship between them. BERT's advantage lies in pre-training on a vast text corpus, followed by fine-tuning for our specific scenario. This process enables BERT to grasp contextual connections between sentences, rendering it effective for tasks like classifying procedures and comprehending the logical flow of information in text. 
% \AF{è basata su GT?}


% \myparagraph{Double Video-Branch for First Mistake Detection}
% \AL{going to fill this once it's clear which is the backbone of PREGO and how it differentiates from OadTR.}




\subsection{Results}
\label{sec:results}

% \FG{In table x we observe that..}

% In Table \ref{tab:together}, we present a detailed summary of the experimental outcomes achieved in our study. It is worth noticing that here the mistakes are categorized as positives.
% (Frequentista è statico, OadTR è limitato dalla finestra temporale. Bert ragiona sullo spazio delle label raggiungendo astrazione maggiore. Prego astrae ancora di più e ha più capacità data il modello grande alla base.)

% The Frequentistic approach yields to results comparable with OadTR in terms of F1-score. However, the former reaches a greater Recall, suggesting that it is able to reduce the False Negatives while the latter catches a smaller number of False Positives. Both methods have some limitations: the first one has a static strategy to determine if an action is a mistake that is strongly related to the training data and the second  has a limited context of the past due to the dimension of the window.
% BERT shows clearly the benefits of including LLM in the anticipation branch: moving the reasoning on an higher abstraction level allows to have more awareness of the past. In this way, BERT possesses the ability to precisely detect the mistakes sacrificing the False Positives. Nevertheless, the Recall indicates that a good number of mistakes are not detected showing a conservative behavior. \LP{sta mettendo molti azioni come non errore, mette l'errore solo se molto certo}
% \LP{mette un buon numero di azioni come errore ed in questo modo riesce a trovarlo quasi sempre}
% PREGO maximize the abstraction level leveraging Symbolic Reasoning with the result that it is able to fully take advantage of the past context information. In this way, it is able to reach the highest F1-score exploiting the ability  to catch all the mistakes. Leveraging DaVinci ..., 




% \FG{this text makes it feel like it's all in table 2, rephrase: "we experimentally evaluate PREGO against the selected baselines on Assembly101-0 and EpicTent-)"}we provide a comprehensive summary of the experimental results obtained in our study.
We experimentally evaluate PREGO against the selected baselines on Assembly101-O and Epic-tent-O. Results are reported in Table \ref{tab:together}

% \FG{I'm doubtful about this sentence.. I tend to believe it's a setup, maybe I'd omit, but I might be wrong. If you feel for it, leave it in, it won't arm}
Considering Assembly101-O, the One-step memory approach achieves results similar to OadTR in terms of F1 score. 
% owever, the former shows a higher Recall, indicating that it can reduce the False Negatives, thus spotting more mistakes. 
%In contrast, the latter reports fewer False Positives, thus avoiding more false alarms. 
% \FG{Somehow this text is not entirely right, since one-step memory is in the label space. Maybe this rephrasing: "
However, both techniques are limited in the length of their temporal dependencies. In fact OadTR is based on processing frames and its performance flattens when surpassing 512 frames (cf.\ Fig.~[3]), only accounting for 64 frames, while procedures last in general 7 minutes. One-step memory reasons on the abstracted label space, where each label summarizes tens of frames. Yet, it only considers the single previous action, which limits its performance.
% "}
% However, both methods have some limitations: the first represents a static strategy to determine if an action is a mistake strongly dependent on the training data, while the second one has a limited context of the past due to the window size.
%\AF{se ho capito bene one-step memory è basata su GT, mentre OadTR no, corretto? Se è così, va detto quando si commentano i risultati.} 

BERT demonstrates the advantages of incorporating LLM in the anticipation branch: by moving the reasoning to a higher level of abstraction, it shows more awareness of the past. In this way, BERT can accurately detect the mistakes by reducing the false alarms. However, the Recall highlights that many mistakes are not detected, revealing a conservative behavior. On the other hand, PREGO maximizes the level of abstraction by leveraging Symbolic Reasoning, enabling it to fully exploit the context information. In this way, it can achieve the highest F1 score demonstrating that symbolic reasoning is a valuable strategy to detect mistakes. Between the two symbolic baselines, namely PREGO$_{Llama}$ and PREGO$_{DaVinci}$, the latter is more capable of producing abstract representation and emerges as the best performer. 

Similar considerations apply to Epic-tent-O with some variations on the scale of the metrics. We attribute these discrepancies to the differences between the two datasets. Indeed, there exist multiple valid procedures for assembling a tent, each dependent on different combinations and orders of actions, whereas industrial assembly processes enforce a stricter among steps as in the case of Assembly101-O. 
% \FG{Change the text here a bit: "
We do not test DaVinci for Epic-tent-O because the processing service is provided at a cost that scales with the number of tokens in input and output, and this is much larger for Epic-tent-O. By contrast LLAMA is open-source and it allows for experimenting on it at scale.
% "}
% On the other hand, LLAMA has open-source policy that allows an illimited number of experiments while DaVinci usage is subjected to varing costs depending on the token number that may reduce its applicability. %\AF{Non menzioniamo le differenze tra Assemble e TENT} \AF{Credo che usiamo Table 2 sia per i main results che per ablation. Forse questa cosa confonde un po', perché quando si arriva qui non è chiaro se abbiamo discusso tutto della tabella o se ci siamo persi qualcosa. Forse possiamo dire in caption che una parte sono risultati e un'altra ablation. Idealmente sarebbe utile avere più tabelle, una per ogni "messaggio" che vogliamo far passare, ma non abbiamo tempo di farlo ora probabilmente.}




% \FG{Attempting to define subsections in this bulleted list:}
% \begin{enumerate}
%     \item Procedural mistake detection. This includes description of baselines, comparison of ours Vs baselines and SOTA, on ASSEMBLY101 and EpicTents, oracle performance of anomaly detection (assuming oracle video recog, or assuming oracle next step?)
%     \item In-depth analysis. This includes video recognition performance of OadTR, next action performance of pattern machines, qualitative, ablative studies \AF{Maybe we could name this section ``Ablation Study'' rather than ``In-depth analysis''. Reviewers are always keen to check boxes and ``Ablation Study'' is a nice box to check :)}
% \end{enumerate}


% \AL{ 
% \begin{itemize}
%     \item Baselines (ours):\begin{itemize}

%         \item{LLM as pattern machines}
%     \end{itemize}
%     \item Baselines (literature):\begin{itemize}
%         \item{\bf Every mistake counts}        
%         \item{\bf POC\cite{POC_2022}}: \AF{we should explain how POC is used for mistake detection, right? Is this an oracle? If so, we should say it (I see it achieves best results)}
%     \end{itemize}
%     \item Datasets: Assembly-101\cite{sener2022assembly101}, Epic-Tent\cite{epicTent}
%     Any results already completed can go in.
% \end{itemize}}



==> sec/Backup/4_exp_2023-11-05.tex <==
\section{Results}
\label{sec:results}
\TD{Detailed list of desired experiments
\begin{itemize}
    \item using bullets
    \item Experiments:
    \item Evaluation metrics:
\end{itemize}}
\AL{ 
\begin{itemize}
    \item Baselines (ours):\begin{itemize}
        \item{\bf Frequentist Baseline}: We define a {\it frequentist transition matrix} considering only the correct procedures. Precisely, given the set of actions in \cite{sener2022assembly101} $\mathcal{T}$ with $|\mathcal{T}|=A$, we define a transition matrix $M\in\mathbb{R}^{A\times A}$ where we annotate the occurrences of the bi-grams of actions in the corrected split of procedures. We then label as {\it mistake} the bi-grams of actions not grounded by the matrix $M$.
        \item{\bf Bayesian Product Ranking}: In addressing the inherent sparsity of the matrix $M$, we draw inspiration from collaborative filtering methods commonly employed in approximating User-Item matrices. We apply the Bayesian Personalized Ranking (BPR)\cite{BPR} as a matrix factorization technique. By considering bi-grams of actions, we fit a BPR model to matrix $M$, interpreting actions as users and items. Given an initial action, the model recommends a top-k list of subsequent actions. An action is deemed \textit{correct} if it naturally follows the initial action and appears in the BPR-recommended list; otherwise, it is marked as a \textit{mistake}. 
        \item{LLM as pattern machines}
        \item{OadTR \cite{OadTR}(green rows in 26.10 meeting, slide 3)}
        \LS{\item {\bf BERT \cite{Devlin2019BERTPO}}: We classify whether procedure B can follow procedure A by using BERT's next sentence prediction (NSP) pre-training task where the model learns to predict whether one sentence naturally follows another in a given text. We refer to procedures as a set of three words e.g. attach wheel chassis, which are coarse actions. You would provide BERT with pairs of procedure A and procedure B sentences as input and ask it to predict whether B follows A. By pre-training BERT on a large corpus of text with the NSP task, it learns to capture contextual relationships between sentences, making it practical for tasks like procedure classification and understanding the logical flow of information in text.}
    \end{itemize}
    \item Baselines (literature):\begin{itemize}
        \item{\bf Every mistake counts}        
        \item{\bf POC\cite{POC_2022}}: 
    \end{itemize}
    \item Datasets: Assembly-101\cite{sener2022assembly101}, Epic-Tent\cite{epicTent}
    Any results already completed can go in.
\end{itemize}}



==> sec/Backup/5_res_27-03.tex <==
\section{Experiments}
\label{sec:experiments}

% \input{Tables/assembly_PREGO}
% \input{Tables/epicTents_PREGO}
% \input{Tables/a101_et}

% \input{Tables/assembly_epic_together}
% \input{Tables/assembly_epic_together_alternative}
% \input{Tables/assembly_epic_together_alternative_2}
\input{Tables/assembly_epic_together_alternative_3}
In this section, we present the results of our experiments on online and open-set mistake detection in procedural videos. We contrast PREGO with several baselines that employ different mistake detector techniques or use the ground truth as an oracle. The oracular scenario represents an upper bound for a given anticipation method since the recognition branch does entirely rely on the ground truth. 
All the baselines are assessed on the \assemblyO and \epicO datasets, detailed in section \ref{sec4:datasets}. The metrics used are precision, recall, and F1 score, explained in \ref{sec4:metrics}. We first describe the baselines in section \ref{sec:baselines}, and then analyze the results in \ref{sec:results}.


\subsection{Baselines}
\label{sec:baselines}

\noindent To estimate the effectiveness of PREGO, we evaluate its performance  by comparing it against the following baseline models based on the metrics presented in Sec.~\ref{sec4:metrics}:

\myparagraph{One-step memory} We define a {\it transition matrix} considering only the correct procedures. Specifically, given the set of the actions  $\mathcal{A}$ in the training set with $|\mathcal{A}|=C$, we define a transition matrix $M\in\mathbb{R}^{C\times C}$ 
which stores in position $(l,m)$ the occurences that action $m$ follows action $l$. 
We then label as {\it mistake} the actions occurring in the test split that do not correspond to transitions recorded in the training set.

\myparagraph{OadTR for mistake detection}
The work~\cite{OadTR} proposes a framework for online action detection called OadTR that employs a Vision Transformer to capture the temporal structure and context of the video clips. The framework consists of an encoder-decoder architecture. The encoder takes the historical observations as input and outputs a task token representing the current action. The decoder takes the encoder output and the anticipated future clips as input and outputs a refined task token incorporating the future context.
% \LP{NEW VERSION:}
% \cite{OadTR} proposes OadTR, a framework for online action detection that employs Transformers to capture the temporal structure and context of the video clips. The framework consists of an encoder-decoder architecture. Drawing inspiration from OadTR, we create a Double-Encoder OadTR that is thought for mistake detection task that is a totally video-based counterpart of PREGO. It employs a dual encoder architecture that performs action recognition in one branch and action prediction in the other. To find if a mistakes is present at time $\bar{\tau}$, the model considers as input the window including the frame to be recognized $f_{\bar{\tau}-w},...,f_{\bar{\tau}}$ in the recognition branch and the same window masked to exclude the current frame $f_{\bar{\tau}-w},...,f_{\bar{\tau}-1}$ in the prediction branch. 
% A discrepancy between the outputs of the encoder and the decoder produces a mistake
In the context of procedural error detection, a mistake is identified when the output from the encoder does not align with the one from the decoder.

\myparagraph{BERT~\cite{Devlin2019BERTPO}}
%\FG{maybe start with "We leverage the capability of BERT and its specific [CLS] token for predicting the correct or mistaken sequence of actions. In more details.." please check this wording}
We leverage the capability of BERT utilizing its specific [CLS] token to predict the correct or erroneous sequence of action. More specifically, we fine-tune BERT using the next-sentence-prediction task, where the model is trained to predict whether one sentence logically follows another within a given text. In our context, we apply this to determine whether step B can follow another step A within a procedure. Here, steps are defined as sets of two words, such as \textit{attach wheel}, representing coarse actions. To perform this, BERT is presented with pairs of sentences corresponding to actions A and B, tasking it with predicting the sequential relationship between them. BERT's advantage lies in pre-training on a vast text corpus, followed by fine-tuning for our specific scenario. This process enables BERT to grasp contextual connections between sentences, rendering it effective for tasks like classifying procedures and comprehending the logical flow of information in text. 


\subsection{Results}
\label{sec:results}
We experimentally evaluate PREGO against the selected baselines on \assemblyO and \epicO.
Results are reported in Table \ref{tab:together}.
Considering \assemblyO, the One-step memory approach achieves results similar to OadTR for MD regarding the F1 score. 
However, both techniques are limited in the length of their temporal dependencies. 
OadTR processes $l$ frames at a time, set to 64 frames by default, while procedures last in general 7 minutes. 
One-step memory reasons on the abstracted label space, where each label summarizes tens of frames. 
However, it only considers the previous action, limiting its performance.
BERT demonstrates the advantages of incorporating LLM in the anticipation branch: moving the reasoning to a higher level of abstraction shows more awareness of the past. 
In this way, BERT can accurately detect the mistakes by reducing the false alarms.
However, the Recall highlights that many mistakes are not detected, revealing a conservative behavior.
On the other hand, PREGO maximizes the level of abstraction by leveraging symbolic reasoning, enabling it to exploit the context information fully. 
In this way, it can achieve the highest F1 score, demonstrating that symbolic reasoning is a valuable strategy to detect mistakes. 
Between the two symbolic baselines, namely PREGO$_{LLama}$ and PREGO$_{DaVinci}$, the latter can produce abstract representation and emerge as the best performer. 

Similar considerations apply to \epicO, with some variations in the scale of the metrics. 
We attribute these discrepancies to the differences between the two datasets. 
Indeed, multiple valid procedures exist for assembling a tent, each dependent on different combinations and orders of action, whereas industrial assembly processes enforce stricter steps, as in the case of \assemblyO. 
\TD{} We do not test DaVinci for Epic-tent-O because the processing service is provided at a cost that scales with the number of tokens in input and output, and this is much larger for \epicO. 
By contrast, LLAMA is open-source, allowing for experimenting on it at scale.

\LS{Added implementation details from supplementary. If we decide to keep them here remove this comment.}
\myparagraph{Implementation Details}
PREGO is trained on two P6000 GPUs using the Adam optimizer, a batch size 128, a learning rate of \(1e^-5\), and a weight decay of \(1e^-4\). 
For Assembly-101-O, we use the pre-extracted TSN frame level features from \cite{sener2022assembly101}. For Epic-Tent-O, we extract the features using the same method. The training process takes approximately 4 hours.

\myparagraph{Speed Analysis}
PREGO achieves 0.02 fps on an NVIDIA Quadro P6000, meeting our needs without real-time constraints. 


% "}
% On the other hand, LLAMA has open-source policy that allows an illimited number of experiments while DaVinci usage is subjected to varing costs depending on the token number that may reduce its applicability. %\AF{Non menzioniamo le differenze tra Assemble e TENT} \AF{Credo che usiamo Table 2 sia per i main results che per ablation. Forse questa cosa confonde un po', perché quando si arriva qui non è chiaro se abbiamo discusso tutto della tabella o se ci siamo persi qualcosa. Forse possiamo dire in caption che una parte sono risultati e un'altra ablation. Idealmente sarebbe utile avere più tabelle, una per ogni "messaggio" che vogliamo far passare, ma non abbiamo tempo di farlo ora probabilmente.}




% \FG{Attempting to define subsections in this bulleted list:}
% \begin{enumerate}
%     \item Procedural mistake detection. This includes description of baselines, comparison of ours Vs baselines and SOTA, on ASSEMBLY101 and EpicTents, oracle performance of anomaly detection (assuming oracle video recog, or assuming oracle next step?)
%     \item In-depth analysis. This includes video recognition performance of OadTR, next action performance of pattern machines, qualitative, ablative studies \AF{Maybe we could name this section ``Ablation Study'' rather than ``In-depth analysis''. Reviewers are always keen to check boxes and ``Ablation Study'' is a nice box to check :)}
% \end{enumerate}


% \AL{ 
% \begin{itemize}
%     \item Baselines (ours):\begin{itemize}

%         \item{LLM as pattern machines}
%     \end{itemize}
%     \item Baselines (literature):\begin{itemize}
%         \item{\bf Every mistake counts}        
%         \item{\bf POC\cite{POC_2022}}: \AF{we should explain how POC is used for mistake detection, right? Is this an oracle? If so, we should say it (I see it achieves best results)}
%     \end{itemize}
%     \item Datasets: Assembly-101\cite{sener2022assembly101}, Epic-Tent\cite{epicTent}
%     Any results already completed can go in.
% \end{itemize}}



==> sec/Backup/main_table.tex <==
% \begin{table*}[t]

% \centering{

% \caption{
% First Mistake Detection (FMD) for PREGO evaluated via F1 score, precision and recall on the Assembly101 and Epic-Tent datasets. \AL{here we're considering TP if a correct action is matched and TN if a mistake action is mismatched.}
% }
% \label{tab:together}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|cc|ccc|cccc} 
% \hline
%  &  &  & \multicolumn{3}{|c|}{\textbf{Assembly101}}  & \multicolumn{3}{c}{\textbf{Epic-Tent}} \\ 


%  & \textbf{Label Space} & \textbf{Frame Space} &\multicolumn{1}{|c}{\textbf{F1 score}} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c|}{\textbf{Recall}}  & \textbf{F1 score} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}} \\ 
% \hline\hline

% \multirow{1}{*}{Frequentist Baseline} & \cmark  & & 83.9 & 85.0 & 82.8 & avoid&this &baseline?\\

% \multirow{1}{*}{Bayesian Personalized Ranking} & \cmark & & 12.7 & 85.0 & 6.8 & 47.7 & 98.4 & 31.5\\

% \multirow{1}{*}{BERT - \cite{Devlin2019BERTPO} for FMD} &  \cmark & &  68.4 & 67.3 & 69.5 &  &  &\\

% \multirow{1}{*}{BERT fine-tuned \cite{Devlin2019BERTPO} for FMD} &  \cmark & & 70.7  & 75.9 &  66.2 &  &  &\\

% \hline

% \multirow{1}{*}{OadTR\cite{OadTR}} &   & \cmark &   &  &  &  &
% &\\



% \multirow{1}{*}{Double Video-Branch for FDM} &   &  \cmark &   & &  &  &
% &\\

% \multirow{1}{*}{PREGO w/ oracle Anticipation} &   & \cmark &   & &  &  &
% &\\

% \multirow{1}{*}{PREGO w/ oracle Recognition} & \cmark  & & 50.0  & 84.2 & 35.6 & 35.8 & 91.9 & 27.4 \\

% \multirow{1}{*}{PREGO} & \cmark & \cmark & 41.3 & 77.5 & 28.2 & 29.9 & 100 & 17.6 \\



% \hline
% \end{tabular}
% }
% }

% \end{table*}


% \begin{table*}[t]

% \centering{

% \caption{
% First Mistake Detection (FMD) for PREGO evaluated via F1 score, precision and recall on the Assembly101 and Epic-Tent datasets.  
% % \AL{here we're considering TN if a correct action is matched and TP if a mistake action is mismatched. I think this is the right way to see it in a mistake detection task.}
% }
% \label{tab:together}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|cc|ccc|cccc} 
% \hline
%  &  &  & \multicolumn{3}{|c|}{\textbf{Assembly101}}  & \multicolumn{3}{c}{\textbf{Epic-Tent}} \\ 


%  & \textbf{Label Space} & \textbf{Frame Space} &\multicolumn{1}{|c}{\textbf{F1 score}} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c|}{\textbf{Recall}}  & \textbf{F1 score} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}} \\ 
% \hline\hline

% \multirow{1}{*}{Frequentist Baseline} & \cmark  & & 21.3 & 16.3 & 30.7 & 10.6 & 6.6 & 26.6\\

% % \multirow{1}{*}{Frequentist Baseline Toy Context} & \cmark  & & 53.69 & 40.92 & 78.02 & 3.9  & 2.7 & 6.6 \\

% \multirow{1}{*}{Bayesian Personalized Ranking} & \cmark & & 46.4 & 30.4 & 98.3 & 17.6 & 9.7 & 93.7 \\

% % \multirow{1}{*}{BERT  \cite{Devlin2019BERTPO} for FMD} &  \cmark & & 10.3 & 10.8 & 9.9   & &  &  &\\


% \multirow{1}{*}{BERT fine-tuned \cite{Devlin2019BERTPO} for FMD} &  \cmark & & 37.6 & 32.8  & 44.0  & 16.2 & 13.6 & 20.0  &\\

% % \multirow{1}{*}{BERT fine-tuned \cite{Devlin2019BERTPO} for FMD- Just 2 examples } &  \cmark & & 41.4 & 44.1  & 39.0  & &  &  &\\

% % \hline

% \multirow{1}{*}{OadTR\cite{OadTR}} &   & \cmark & ON   & ON  & ON & ON  & ON & ON\\



% % \multirow{1}{*}{Double Video-Branch for FDM} &   &  \cmark &   & &  &  & &\\

% % \multirow{1}{*}{PREGO w/ oracle Anticipation} &   & \cmark &   & &  &  &
% % &\\

% \multirow{1}{*}{PREGO w/ oracle Recognition} & \cmark & & 42 & 26.9 & 95.5  & 20.6 & 11.45 & 100 \\

% \multirow{1}{*}{PREGO} & \cmark & \cmark & 33.4 & 20.4 & 91.7 & 13.8 & 7.54 & 80.0 \\



% \hline
% \end{tabular}
% }
% }

% \end{table*}

\begin{table*}[t]

\centering{

\caption{
A comparative assessment between PREGO and the chosen baseline methods is conducted on the task of detecting procedural mistakes using the Assembly101-O and Epic-Tent-O datasets. The initial section of the table, highlighted in grey, focuses on Oracle Recognition.
}
% \FG{I cannot see a good reason for not having reported prego-llama-13B on epic-tent-O. If we don't get it in time, then leave the line out and we include it in the supp mat when we get it next week. Btw 31.2 is also not 100\% a convincing number}}
% \FG{Consider this rephrasing: "Comparative evaluation of PREGO Vs the selected baselines on the task of procedural mistake detection on the Assembly101-O and Epic-Tent-O datasets". Also place the oracular PREGO performance below, after a bar, as it's not comparable with others.} First Mistake Detection (FMD) for PREGO evaluated via F1 score, precision and recall on the Assembly101 and Epic-Tent datasets.}  
% \AL{here we're considering TN if a correct action is matched and TP if a mistake action is mismatched. I think this is the right way to see it in a mistake detection task.}
% \LP{Agree with Ale and I suppose it would be better to state it cleearly to avoid confusion in the interpretation}

% \label{tab:together}
% \resizebox{0.85\linewidth}{!}{
% \begin{tabular}{l|ccc|cccc} 
% \hline
%  & \multicolumn{3}{|c|}{\textbf{Assembly101-O}}  & \multicolumn{3}{c}{\textbf{Epic-Tent-O}} \\ 


%  & \multicolumn{1}{|c}{\textbf{F1 score}} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c|}{\textbf{Recall}}  & \textbf{F1 score} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}} \\ 
% \hline\hline

% \multirow{1}{*}{One-step memory} &  21.3 & 16.3 & 30.7 & 10.6 & 6.6 & 26.6\\

% % \multirow{1}{*}{Frequentist Baseline Toy Context} & \cmark  & & 53.69 & 40.92 & 78.02 & 3.9  & 2.7 & 6.6 \\

% % \multirow{1}{*}{Bayesian Personalized Ranking} & 31.2 & 21.7 & 55.1 & 16.7 & 9.2 & 93.3 \\
% %& 17.6 & 9.7 & 93.7

% % \multirow{1}{*}{BERT  \cite{Devlin2019BERTPO} for FMD} &  \cmark & & 10.3 & 10.8 & 9.9   & &  &  &\\


% % \multirow{1}{*}{BERT fine-tuned \cite{Devlin2019BERTPO} for FMD} &  \cmark & & 37.6 & 32.8  & 44.0  & 16.2 & 13.6 & 20.0  &\\


% \multirow{1}{*}{OadTR for MD\cite{OadTR}}  & 20.7   & 24.3  & 18.1 & 10.2  & 6.7 & 21.7\\


% \multirow{1}{*}{BERT \cite{Devlin2019BERTPO}} & 31.8 & 78.2  & 20.0  & 10.4 & 75.0 & 5.6  &\\


% % \multirow{1}{*}{BERT fine-tuned \cite{Devlin2019BERTPO} for FMD- Just 2 examples } &  \cmark & & 41.4 & 44.1  & 39.0  & &  &  &\\

% % \hline




% % \multirow{1}{*}{Double Video-Branch for FDM} &   &  \cmark &   & &  &  & &\\

% % \multirow{1}{*}{PREGO w/ oracle Anticipation} &   & \cmark &   & &  &  &
% % &\\



% \multirow{1}{*}{PREGO_\textit{(LLAMA)} - OadTR} & 33.4 & 20.4 & 91.7 & 13.8 & 7.54 & 80.0 \\
% % \multirow{1}{*}{PREGO\textit{_{(LLAMA-13B)}}} & 31.2 & 19.1 & 84.0 & - & - & - \\
% \multirow{1}{*}{PREGO_\textit{(DaVinci)} - OadTR} & 35.8 & 22.1 & 94.2 & - & - & - \\
% \multirow{1}{*}{PREGO_\textit{(LLAMA)} - MiniROAD} & 35.8 & 22.1 & 94.2 & - & - & - \\


% \hline

% \multirow{1}{*}{\textcolor{gray}{PREGO_\textit{(LLAMA)} - oracle Recognition}} & \textcolor{gray}{42.0} & \textcolor{gray}{26.9} & \textcolor{gray}{95.5}  & \textcolor{gray}{20.6} & \textcolor{gray}{11.45} & \textcolor{gray}{100} \\
% % \multirow{1}{*}{\textcolor{gray}{PREGO\textit{_{(LLAMA-13B)}} - oracle Recognition}} & \textcolor{gray}{44.1} & \textcolor{gray}{28.5} & \textcolor{gray}{97.8}  & \textcolor{gray}{-} & \textcolor{gray}{-} & \textcolor{gray}{-} \\

% \multirow{1}{*}{\textcolor{gray}{PREGO_\textit{(DaVinci)} - oracle Recognition}} & \textcolor{gray}{46.3} & \textcolor{gray}{30.6} & \textcolor{gray}{94.3 }  & \textcolor{gray}{-} & \textcolor{gray}{-} & \textcolor{gray}{-} \\

   
% \hline
% \end{tabular}
% }
% }

% \end{table*}





\label{tab:together}
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{l|ccc|cccc} 
\hline
 & \multicolumn{3}{|c|}{\textbf{Assembly101-O}}  & \multicolumn{3}{c}{\textbf{Epic-Tent-O}} \\ 


 & \multicolumn{1}{|c}{\textbf{F1 score}} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c|}{\textbf{Recall}}  & \textbf{F1 score} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}} \\ 
\hline\hline

\multirow{1}{*}{\textcolor{gray}{One-step memory -oracleRecognition}} &  \textcolor{gray}{21.3} & \textcolor{gray}{16.3} & \textcolor{gray}{30.7} & \textcolor{gray}{10.6} & \textcolor{gray}{6.6} & \textcolor{gray}{26.6}\\

\multirow{1}{*} {\textcolor{gray}{{BERT \cite{Devlin2019BERTPO}} - oracleRecognition}} & \textcolor{gray}{31.8} & \textcolor{gray}{78.2}  & \textcolor{gray}{20.0}  & \textcolor{gray}{10.4} & \textcolor{gray}{75.0} & \textcolor{gray}{5.6}  &\\

\multirow{1}{*}{\textcolor{gray}{PREGO_\textit{(LLAMA)} - oracle Recognition}} & \textcolor{gray}{42.0} & \textcolor{gray}{26.9} & \textcolor{gray}{95.5}  & \textcolor{gray}{20.6} & \textcolor{gray}{11.45} & \textcolor{gray}{100} \\

\multirow{1}{*}{\textcolor{gray}{PREGO_\textit{(DaVinci)} - oracle Recognition}} & \textcolor{gray}{46.3} & \textcolor{gray}{30.6} & \textcolor{gray}{94.3 }  & \textcolor{gray}{-} & \textcolor{gray}{-} & \textcolor{gray}{-} \\

\hline


\multirow{1}{*}{OadTR for MD~\cite{OadTR}}  & 20.7   & 24.3  & 18.1 & 10.2  & 6.7 & 21.7\\



% \multirow{1}{*}{PREGO_\textit{(LLAMA)} - OadTR} & 33.4 & 20.4 & 91.7 & 13.8 & 7.54 & 80.0 \\
% % \multirow{1}{*}{PREGO\textit{_{(LLAMA-13B)}}} & 31.2 & 19.1 & 84.0 & - & - & - \\
% \multirow{1}{*}{PREGO_\textit{(DaVinci)} - OadTR} & 35.8 & 22.1 & 94.2 & - & - & - \\

\multirow{1}{*}{PREGO_\textit{(LLAMA)} - MiniRoad~\cite{An2023MiniROADMR}} & 35.8 & 22.1 & 94.2 & - & - & - \\

\multirow {1}{*}{PREGO_\textit{(DaVinci)} - MiniRoad~\cite{An2023MiniROADMR}} & - & - & - & - & - & - \\

\hline



   
\hline
\end{tabular}
}
}

\end{table*}

==> sec/Backup/main_table_27-03.tex <==
% \begin{table*}[t]

% \centering{
%     \caption{
%         A comparative assessment between PREGO and the chosen baseline methods is conducted on the task of detecting procedural mistakes using the Assembly101-O and Epic-Tent-O datasets. 
%         $\dagger$ means the model receives ground truth actions rather than those predicted by the step recognizer.
%         % makes Oracle Recognition less explicit and removes Step recog. columns
%     }
%     \label{tab:together}
%     \resizebox{0.85\linewidth}{!}{
%         \begin{tabular}{l|c|ccc|ccc} 
        
%          & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{3}{c|}{\textbf{Assembly101-O}}  & \multicolumn{3}{c}{\textbf{Epic-Tent-O}} \\ 
%          & \multicolumn{1}{c|}{\textbf{Step Recog.}} &  \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}}  & \multicolumn{1}{c|}{\textbf{F1 score}} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}} & \multicolumn{1}{c}{\textbf{F1 score}}\\ 
%         \hline\hline
%         \multirow{1}{*}{One-step memory} & - & 16.3 & 30.7 & 21.3 & 6.6 & av.6 & 10.6\\
%         \multirow{1}{*}{BERT \cite{Devlin2019BERTPO}} & - &  78.2  & 20.0  & 31.8 & 75.0 & 5.6 & 10.4\\
%         \multirow{1}{*}{OadTR for MD~\cite{OadTR}}  & - &  24.3  & 18.1 & 20.7   & 6.7 & 21.7 & 10.2\\
%         % \multirow{1}{*}{PREGO_\textit{(LLAMA)} - OadTR} &  20.4 & 91.7 & 33.4 & 7.54 & 80.0 & 13.8\\
%         % % \multirow{1}{*}{PREGO\textit{_{(LLAMA-13B)}}} & 31.2 & 19.1 & 84.0 & - & - & - \\
%         % \multirow{1}{*}{PREGO_\textit{(DaVinci)} - OadTR} & 35.8 & 22.1 & 94.2 & - & - & - \\
%         \multirow{1}{*}{PREGO_\textit{LLAMA}} & OadTR~\cite{OadTR} & 22.1 & 94.2 & 35.8 & 7.1 & 73.3 & 12.9 \\
%         \multirow{1}{*}{PREGO_\textit{LLAMA}} & MiniRoad~\cite{An2023MiniROADMR} & 28.0 & 71.4 & 40.0 & 6.6 & 53.3 & 11.7 \\
%         \multirow {1}{*}{PREGO_\textit{DaVinci}} & MiniRoad~\cite{An2023MiniROADMR} & - & - & - & - & - & - \\ 
%        \multirow{1}{*}{PREGO_\textit{LLAMA}} & - & 26.9 & 95.5 & 42.0 & 11.45 & 100 & 20.6 \\
%         \multirow{1}{*}{PREGO_\textit{DaVinci}} & - & 30.6 & 94.3 & 46.3 & - & - & - \\
%         \hline
%         \end{tabular}
%     }
% }

% \end{table*}

\begin{table*}[t]

\centering{
    \caption{
        A comparative assessment between PREGO and the chosen baseline methods is conducted on the task of detecting procedural mistakes using the \assemblyO and \epicO datasets. \LS{Should we distinguish the actual PREGO (LLAMA + MiniRoad)}
        % $\dagger$ means the model receives ground truth actions rather than those predicted by the step recognizer.
        % makes Oracle Recognition less explicit and removes Step recog. columns
    }
    \label{tab:together}
    \resizebox{0.85\linewidth}{!}{
        \begin{tabular}{l|c|c|ccc|ccc} 
        
         & \multicolumn{2}{c|}{\textbf{}} & \multicolumn{3}{c|}{\textbf{\assemblyO}}  & \multicolumn{3}{c}{\textbf{\epicO}} \\ 
         & \multicolumn{1}{c|}{\textbf{Step Recog.}} & \multicolumn{1}{c|}{\textbf{Step Antic.}} &  \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}}  & \multicolumn{1}{c|}{\textbf{F1 score}} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}} & \multicolumn{1}{c}{\textbf{F1 score}}\\ 
        \hline\hline
        \multirow{1}{*}{One-step memory} &  \textit{\textcolor{gray}{Oracle}} & \xmark & 16.3 & 30.7 & 21.3 & 6.6 & 26.6 & 10.6\\
        \multirow{1}{*}{BERT \cite{Devlin2019BERTPO}} &  \textit{\textcolor{gray}{Oracle}} & \xmark & 78.2  & 20.0  & 31.8 & 75.0 & 5.6 & 10.4\\
        \multirow{1}{*}{OadTR for MD~\cite{OadTR}}  &  \textit{OadTR~\cite{OadTR}} &  \textit{OadTR~\cite{OadTR}} & 24.3  & 18.1 & 20.7   & 6.7 & 21.7 & 10.2\\
        % \multirow{1}{*}{PREGO_\textit{(LLAMA)} - OadTR} &  20.4 & 91.7 & 33.4 & 7.54 & 80.0 & 13.8\\
        % % \multirow{1}{*}{PREGO\textit{_{(LLAMA-13B)}}} & 31.2 & 19.1 & 84.0 & - & - & - \\
        % \multirow{1}{*}{PREGO_\textit{(DaVinci)} - OadTR} & 35.8 & 22.1 & 94.2 & - & - & - \\
        \multirow{1}{*}{\textit{PREGO}} &   \textit{OadTR~\cite{OadTR}} &  \textit{LLAMA} & 22.1 & 94.2 & 35.8 & 7.1 & 73.3 & 12.9 \\
        \multirow{1}{*}{\textit{PREGO}} &  \textit{MiniRoad~\cite{An2023MiniROADMR}} &  \textit{LLAMA} & 28.0 & 71.4 & 40.0 & 6.6 & 53.3 & 11.7 \\
        \multirow {1}{*}{\textit{PREGO}} &  \textit{MiniRoad~\cite{An2023MiniROADMR}} &  \textit{DaVinci} & - & - & - & - & - & - \\ 
        \hline
       \multirow{1}{*}{\textit{PREGO}} & \textit{\textcolor{gray}{Oracle} }&  \textit{LLAMA} & 26.9 & 95.5 & 42.0 & 11.45 & 100 & 20.6 \\
        \multirow{1}{*}{\textit{PREGO}} & \textit{\textcolor{gray}{Oracle}} &   \textit{DaVinci}  & 30.6 & 94.3 & 46.3 & - & - & - \\
        \hline
        \end{tabular}
    }
}

\end{table*}
